Fully Adaptive Composition in Differential Privacy

Composition is a key feature of differential privacy. Well-known advanced composition theorems allow one to query a private database quadratically more times than basic privacy composition would permit. However, these results require that the privacy parameters of all algorithms be fixed before interacting with the data. To address this, Rogers et al. introduced fully adaptive composition, wherein both algorithms and their privacy parameters can be selected adaptively. They defined two probabilistic objects to measure privacy in adaptive composition: privacy filters, which provide differential privacy guarantees for composed interactions, and privacy odometers, time-uniform bounds on privacy loss. There are substantial gaps between advanced composition and existing filters and odometers. First, existing filters place stronger assumptions on the algorithms being composed. Second, these odometers and filters suffer from large constants, making them impractical. We construct filters that match the rates of advanced composition, including constants, despite allowing for adaptively chosen privacy parameters. En route we also derive a privacy filter for approximate zCDP. We also construct several general families of odometers. These odometers match the tightness of advanced composition at an arbitrary, preselected point in time, or at all points in time simultaneously, up to a doubly-logarithmic factor. We obtain our results by leveraging advances in martingale concentration. In sum, we show that fully adaptive privacy is obtainable at almost no loss.

==> Old_Tex/FilterOLD.tex <==
\section{A Filter That Matches Advanced Composition}
\label{sec:filter}
In this section, we show that the same rate as advanced composition can be achieved under the assumption that the algorithms being composed are conditionally probabilistically differentially private. In particular, using the terminology of Section~\ref{sec:martingales:ploss}, we construct a privacy filter such that, when the privacy parameters are fixed in advance, we recover the rate as advanced composition. Our privacy filter greater improves on the rate of the original filter presented in \cite{rogers2016odometer}, and matches the rate of the Renyi filter presented in \cite{feldman2020individual}. However, we can prove the validity of our filter without under-the-hood conversions between differential privacy, zero-concentrated differential privacy \cite{balsubramani2014sharp}, and Renyi differential privacy \cite{mironov2017renyi}, offering a more straightforward proof using the time-uniform bounds presented in \cite{howard2020line}.

While in this section we still require that the algorithms being composed are conditionally probabilistically differentially private (which is a stronger assumption than just conditional differential privacy), in the next section we show how to remove this assumption. This in turn allows us to exactly match the rate of advanced composition while allowing privacy parameters to be adaptively selected.

We now state the main result of this section.

\begin{theorem}
\label{thm:new_filter}
Suppose $(A_n)_{n \in \N}$ is a sequence of algorithms, $\{(\calF_n(x))_{n \in \N}\}_{x \in \calX}$ a collection of filtrations, and $\{(\epsilon_n(x), \delta_n(x))_{n \in \N}\}_{x \in \calX}$ a collection of privacy paramters such that $A_n$ is $(\epsilon_n, \delta_n)$-pDP conditioned on $\calF_{n - 1}$, for all $n \in \N$. Let $\epsilon > 0$ be a target privacy parameter, and $\delta = \delta' + \delta''$ a target approximation parameter such that $\delta' > 0, \delta'' \geq 0$. For any $x \in \calX$, define the $(\calF_n(x))_{n \in \N}$-stopping time $N(x)$ by
$$
N(x) := \inf\left\{n \in \N : \epsilon < \sqrt{2\log\left(\frac{1}{\delta'}\right)\sum_{m \leq n + 1}\epsilon_m(x)^2} + \frac{1}{2}\sum_{m \leq n + 1}\epsilon_m(x)^2\right\} \wedge \inf\left\{n \in \N : \delta'' <  \sum_{m \leq n + 1}\delta_m(x)\right\},
$$
where $a \land b := \min\{a, b\}$. Then, the collection of stopping times $\{N(x)\}_{n \in \N}$ form an $(\epsilon, \delta)$-privacy filter.
\end{theorem}

For now, we hold off on the proof of Theorem~\ref{thm:new_filter} to make several observations. First, assume that the sequence of privacy parameters are fixed in advance, i.e. $\epsilon_n(x) := \epsilon_n$ and $\delta_n(x) := \delta_n$ are constants independent of choice of database $x \in \calX$. Then, for any $\delta' > 0$, taking $\epsilon := \sqrt{2\log\left(\frac{1}{\delta'}\right)\sum_{m \leq n}\epsilon_m^2} + \frac{1}{2}\sum_{m \leq n}\epsilon_m^2$ and $\delta'' := \sum_{m \leq n}\delta_m$ exactly recovers the rate of advanced composition. Second, note that while we do define a separate stopping time for each $x \in \calX$, all stopping times on depend on the underlying private database through the sequence of privacy parameters being chosen. Hence, while the underlying databases are unknown in general, the stopping conditions are readily computable.

Now, we proceed to the proof of Theorem~\ref{thm:new_filter}. Before we can get started, we need to following bound of the conditional expectation of privacy loss, which can be immediately obtained from the bound on expected privacy loss presented in \cite{bun2016concentrated}.

\begin{lemma}
\label{lem:priv_loss_bound}
Suppose $A$ is algorithm, $\{\calH(x)\}_{x \in \calX}$ a collection of $\sigma$-algebras, and $\{\epsilon(x)\}_{x \in \calX}$ a collection of privacy parameters such that $A$ is $(\epsilon, 0)$-pDP conditioned on $\calH$. Then, for any input dataset $x \in \calX$ and neighboring dataset $x' \sim x \in \calX$, we have that
$$
\E\left(\calL(x, x') | \calH(x)\right) \leq \frac{1}{2}\epsilon^2.
$$
\end{lemma}

Now, we prove Theorem~\ref{thm:new_filter}.

\begin{proof}[\textbf{Proof of Theorem~\ref{thm:new_filter}}]
To begin, we assume that the algorithms $(A_n)$ satisfying $(\epsilon_n, 0)$-pDP conditionede on $\calF_{n - 1}$. We will show how to alleviate this assumption in the second half of the proof. Fix an input database $x \in \calX$. Recall that we have already argued that, for any neighboring dataset $x' \sim x \in \calX$, the process
$$
M_n := M_n(x, x') = \calL_{1:n}(x, x') - \sum_{m \leq n}\E\left(\calL_m(x, x') | \calF_{n - 1}(x)\right)
$$
is a martingale with respect to $(\calF_n(x))_{n \in \N}$ and that its increments $\Delta M_n := \calL_n(x, x') - \E\left(\calL_n(x, x')|\calF_{n - 1}(x)\right)$ are $\epsilon_n(x)^2$-subGaussian conditioned on $\calF_{n - 1}(x)$.

Thus, by Fact~\ref{fact:line_cross}, we know that, for any $b, a > 0$, we have
$$
\P\left(\exists n \in \N : M_n \geq \frac{b}{2} + \frac{b}{2a}V_n(x)\right) \leq \exp\left(\frac{-b^2}{2a}\right),
$$
where the process $(V_n(x))_{n \in \N}$ given by $V_n(x) := \sum_{m \leq n}\epsilon_m(x)^2$ is the accumulated variance up to and including time $n$. Thus, it suffices to optimize the free parameters $b$ and $a$ to prove the result.

To do this, consider the following function $f : \R_{\geq 0} \rightarrow \R_{\geq 0}$ given by
$$
f(y) = \sqrt{2\log\left(\frac{1}{\delta'}\right)y} + \frac{1}{2}y.
$$
Clearly, $f$ is a quadratic in $\sqrt{y}$ which is strictly increasing. In particular, one can readily check that 
$$
y^\ast :=  \left(-\sqrt{2\log\left(\frac{1}{\delta'}\right)} + \sqrt{2\log\left(\frac{1}{\delta'}\right) + \epsilon}\right)^2
$$
solves the equation $f(y) = \epsilon$, where $\epsilon > 0$ is the target privacy parameter. 

As such, setting $a := y^\ast$ and $b := \sqrt{2\log\left(\frac{1}{\delta'}\right)y^\ast}$ yields
$$
\exp\left(\frac{-b^2}{a}\right) = \exp\left(\frac{2y^\ast\log\left(\frac{1}{\delta'}\right)}{y^\ast}\right) = \delta'.
$$

Furthermore, expanding the definition of $(M_n)_{n \in \N}$, the parameters yield, for any $n \leq N(x)$:
\begin{align*}
\calL_{1:n}(x, x') &\leq \frac{b}{2} + \frac{b}{2a}V_n + \sum_{m \leq n}\E\left(\calL_m(x, x') \mid \calF_{m - 1}(x)\right) \leq \frac{b}{2} + \frac{b}{2a}\sum_{m \leq n}\epsilon_m(x)^2 + \frac{1}{2}\sum_{m \leq n}\epsilon_m(x)^2\\
&= \frac{1}{2}\sqrt{2\log\left(\frac{1}{\delta'}\right)y^\ast} + \frac{1}{2}\frac{\sqrt{2\log\left(\frac{1}{\delta'}\right)y^\ast}}{y^\ast}\sum_{m \leq n}\epsilon_m(x)^2 + \frac{1}{2}\sum_{m \leq n}\epsilon_m(x)^2 \\
&\leq \frac{1}{2}\sqrt{2\log\left(\frac{1}{\delta'}\right)y^\ast} + \frac{1}{2}\sqrt{2\log\left(\frac{1}{\delta'}\right)y^\ast} + \frac{1}{2}\sum_{m \leq n}\epsilon_m(x)^2 \\
&= \sqrt{2\log\left(\frac{1}{\delta'}\right)y^\ast} + \frac{1}{2}\sum_{m \leq n}\epsilon_m(x)^2 \leq \sqrt{2\log\left(\frac{1}{\delta'}\right)y^\ast} + \frac{1}{2}y^\ast = \epsilon.
\end{align*}
Thus, we have proven the desired result in the case where all algorithms have $\delta_n(x) = 0$.

Now, we show how to generalize our result to the case where the approximation parameters $\delta_n(x)$ are not identically zero. Define the events
$$
A := \left\{\exists n \leq N(x) : \calL_{1:n}(x, x') > \epsilon\right\} \qquad \text{and} \qquad B := \left\{\exists n \leq N(x): \calL_n(x, x') > \epsilon_n(x)\right\}.
$$
Our goal is to show that, with $N(x)$ defined as in the statement of Theorem~\ref{thm:new_filter}, that $\P(A) \leq \delta$. Simply using Bayes rule, we have that
$$
\P(A) = \P(A \cap B^c) + \P(A \cap B) \leq \P(A|B^c) + \P(B) \leq \delta' + \P(B),
$$
where the third inequality follows from our already-completed analysis in the case that $\delta_n = 0$. Now, we show that $\P(B) \leq \delta''$, which suffices to prove the result as we have, by assumption, $\delta = \delta' + \delta''$. 

Define the modified privacy loss random variables $(\widetilde{\calL}_n(x, x'))_{n \in \N}$ by
$$
\widetilde{\calL}_n(x, x') := \begin{cases} \calL_n(x, x') \qquad n \leq N(x) \\
0 \qquad \text{otherwise}
\end{cases}.
$$
Likewise, define the modified privacy parameter random variables $\widetilde{\epsilon}_n(x)$ and $\widetilde{\delta}_n(x)$ in an identical manner. Then, we can bound $\P(B)$ in the following manner:
\begin{align*}
    \P(\exists n \leq N(x) : \calL_n(x, x') > \epsilon_n(x)) &= \P\left(\exists n \in \N : \widetilde{\calL}_n(x, x') > \widetilde{\epsilon}_n(x)\right) \\
    &\leq \sum_{n = 1}^\infty \P\left(\widetilde{\calL}_n(x, x') > \widetilde{\epsilon}_n(x) \right) = \sum_{n = 1}^\infty \E\P\left(\widetilde{\calL}_n(x, x') > \widetilde{\epsilon}_n(x) | \mathcal{F}_{n- 1}(x)\right)\\
    &\leq \sum_{n = 1}^\infty \E\widetilde{\delta}_n(x) = \E\left[\sum_{n = 1}^\infty \widetilde{\delta}_n(x)\right] =\mathbb{E}\left[\sum_{n \leq N(x)}\delta_n(x)\right] \leq \delta''.
\end{align*}
Thus, we have have proven the desired result in the general case, and are done.


\end{proof}

Note that the identical result can be obtained leveraging in the analysis for Renyi filters presented in \cite{feldman2020individual}. However, our approach has the advantage that it does not leverage any block box reductions between different modes of privacy, simply building off of line-crossing inequalities for martingales.


==> Old_Tex/FullyAdaptive.tex <==
\section{Fully Adaptive Composition}
\label{sec:fully_adaptive}

In the previous section, we demonstrated how to match the composition rate of advanced composition under the assumption that the algorithms beings composed satisfy conditional probabilistic differential privacy. As noted in Lemma~\ref{lem:dp_to_pdp}, there is in fact a gap between probabilistic differential privacy and (standard) differential privacy: all algorithms that satisfy probabilistic differential privacy also satisfy differential privacy, but the converse is not true. Instead, a potentially costly conversion is required to make a general differentially private algorithm probabilistically differentially private. In order to prove our results in Section~\ref{sec:filter}, we needed to assume that the algorithms being composed satisfies pDP. In this section, we demonstrate that our results in Section~\ref{sec:filter} actually hold under the weaker assumption that the algorithms being composed satisfy conditional differential privacy, avoiding the conversion costs that were necessary in other works \cite{rogers2016odometer, feldman2020individual}.


In short, our goal in this section is to prove the following theorem.

\begin{theorem}
\label{thm:fully_adaptive}
Suppose $(A_n)_{n \geq 1}$ is a sequence of algorithms and $(B_n)_{n \geq 1}$ a sequence of post-processing algorithms, as outlined in Section~\ref{sec:background:dp}. Suppose, for any $n \geq 1$, that $A_n$ is $(\epsilon_n, \delta_n)$-differentially private conditioned on $(A_{1:n-1}, B_{1:n -1})$. Let $\epsilon > 0$ be a target privacy parameter, and $\delta = \delta' + \delta''$ a target approximation parameter such that $\delta' > 0, \delta'' \geq 0$. Consider the function $N : \R_{\geq 0}^\infty \times \R_{\geq 0}^\infty \rightarrow \N$ given by
$$
N((\epsilon_n)_{n \in \N}, (\delta_n)_{n \in \N}) := \inf\left\{n \in \N : \epsilon < \sqrt{2\log\left(\frac{1}{\delta'}\right)\sum_{m \leq n + 1}\epsilon_m^2} + \frac{1}{2}\sum_{m \leq n + 1}\epsilon_m^2\right\} \wedge \inf\left\{n \in \N : \delta'' <  \sum_{m \leq n + 1}\delta_m\right\},
$$
where $a \land b := \min\{a, b\}$. Then, the algorithm $A_{1:N(\cdot)}(\cdot) : \calX \rightarrow \calY^\infty$ is $(\epsilon, \delta)$-differentially private, where $N(x) := N((\epsilon_n(x))_{n \geq 1}, (\delta_n(x))_{n \geq 1})$.
\end{theorem}

The statement of Theorem~\ref{thm:fully_adaptive} appears essentially the same as Theorem~\ref{thm:new_filter}. However, there are two differences. First, as mentioned in the previous paragraph, we loosen the assumption of conditional probabilistic differential privacy to that of just conditional differential privacy. Secondly, we only claim that the composed algorithm is $(\epsilon, \delta)$-differentially private. In particular, we make no claims about the privacy loss of the composed interaction. This is because, in general, probabilistic differential privacy and differential privacy are \textit{not} equivalent, per Lemma~\ref{lem:dp_to_pdp}. 

It turns out that in order to prove Theorem~\ref{thm:fully_adaptive}, we need some additional machinery. In particular, we need to briefly study and generalize what is perhaps the simplest example of a differentially private algorithm: randomized response. The setup for randomized response is simple. The space of datasets is simply $\{0, 1\}$, i.e. a dataset consists of a single hidden bit. The mechanism works as follows. With some small probability, the algorithm fully reveals the hidden bit, either by revealing the symbol $\top$ for $1$ or $\bot$ for $0$. Otherwise, the algorithm flips a slightly biased coin, keeping the hidden bit the same with some probability, and flipping the bit with some comparable but smaller probability. 

\begin{definition}[Randomized Response]
\label{def:rr}
Let $\calR := \{0, 1, \top, \bot\}$ and $2^\calR$ the corresponding power set of $\calR$. Then, an algorithm $R$ taking inputs in $\{0, 1\}$ to outputs in the measurable space $(\calR, 2^\calR)$ is said to be an instance of $(\epsilon, \delta)$-randomized response if $R(b)$ has the following distribution.
$$
R(b) = \begin{cases} b  &\text{with probability } (1 - \delta)\frac{e^\epsilon}{1 + e^\epsilon} \\
1 - b &\text{with probability } (1 - \delta)\frac{1}{1 + e^\epsilon}\\
\top &\text{with probability } \delta \text{ if } b = 1\\
\bot &\text{with probability } \delta \text{ if } b = 0.
\end{cases}
$$
\end{definition}
The following two facts about randomized response can be easily checked:
\begin{itemize}
    \item $(\epsilon, \delta)$-randomized response satisfies $(\epsilon, \delta)$-DP.
    \item $(\epsilon, \delta)$-randomized response also satisfies $(\epsilon, \delta)$-pDP.
\end{itemize}
The fact that it satisfies probabilistic differential privacy at no loss, that is with the same parameters, will be crucial later on. The last important, and possibly surprising, fact is that \textit{any} $(\epsilon, \delta)$-DP algorithm can be viewed as a randomized post-processing of randomized response \cite{kairouz2015composition, murtagh2016complexity}, as formalized below. 

\begin{lemma}[Reduction to Randomized Response \cite{kairouz2015composition}]
\label{fact:post_proc_rr}
Let $A$ be a $(\epsilon, \delta)$-differentially private algorithm taking inputs from $\calX$ to some measurable space $(\calY, \calG)$. Let $R$ be an instance of $(\epsilon, \delta)$-randomized response. Then, for any input dataset $x_0 \in \calX$ and any neighboring dataset $x_1 \sim x_0$, there is a transition kernel $\nu : \calG \times \calR \rightarrow [0,1]$ such that 
$\P(A(x_b) \in \cdot ) = \nu_b$, where $\nu_b  = \E \nu(\cdot, R(b))$\footnote{By $\nu_b(\cdot) := \E \nu(\cdot, R(b))$, we mean $\nu_b$ is the averaged probability measure given by $$\nu_b(\cdot) = \P(R(b) = 1)\nu(\cdot, 1) + \P(R(b) = 0)\nu(\cdot, 0) + \P(R(b) = \bot)\nu(\cdot, \bot) + \P(R(b) = \top)\nu(\cdot, \top).$$}.

\end{lemma}


Lemma~\ref{fact:post_proc_rr} is a very powerful result --- in fact it can be used to prove advanced composition \cite{kairouz2015composition}. However, we need a slightly more detailed result to hold. This is because we want to allow privacy parameters to be adaptively selected over time. To facilitate a generalization, we first describe a generalization of randomized response to a conditional setting --- that is a setting wherein the parameters $\epsilon$ and $\delta$ associated with randomized response can be selected according to some auxiliary information. We define conditional randomized response as follows.

\begin{definition}[Conditional Randomized Response]
\label{def:cond_rr}
Let $R$ be an algorithm taking inputs in $\{0, 1\}$ to outputs in the measurable space $(\calR, 2^\calR)$, and let $B$ be an algorithm taking inputs in $\{0, 1\}$ to outputs in $(\calZ, \calH)$. For functions $\epsilon, \delta : \calZ \rightarrow \R_{\geq 0}$, we say $R$ is an instance of $(\epsilon, \delta)$-randomized response conditioned on $B$ if, for all $b, b' \in \{0, 1\}$, on the event $\{B(b') = z\}$, the conditional probability $\P(R(b) \in \cdot | B(b'))$ is equivalent to the law of $(\epsilon(z), \delta(z))$-randomized response with input bit $b$, per Definition~\ref{def:rr}.
\end{definition}

Definition~\ref{def:cond_rr}, heuristically, tells us that once we observe that random variable $B$ yields some value $z \in \calZ$, the conditional laws of $R(0)$ and $R(1)$ just become that of regular randomized response with some known privacy parameters $\epsilon(z)$ and $\delta(z)$. Using the above generalization of randomized response, we can formulate a conditional analogue of Lemma~\ref{fact:post_proc_rr}. 

\begin{lemma}[Reduction to Conditional Randomized Response]
\label{lem:cond_post_rr}
Let $A$ and $B$ be algorithms taking inputs in $\calX$ to outputs in a measurable spaces $(\calY, \calG)$ and $(\calZ, \calH)$ respectively. Suppose $A$ is $(\epsilon, \delta)$-differentially private conditioned on $B$. Fix an input $x_0 \in \calX$ and a neighboring dataset $x_1 \sim x_0$. Let $R$ be an instance of $(\epsilon, \delta)$-randomized response conditioned on $B(x_{(\cdot)})$ (where $x_{(\cdot)}$ indicates a placeholder for a bit in $\{0, 1\}$). Then, there is a transition kernel $\nu : \calG \times \calR \times \calZ \rightarrow [0, 1]$ such that, for all $b, b' \in \{0, 1\}$, $\P\left(A(x_b) \in \cdot | B(b')\right) = \nu_{b, b'}$, where $\nu_{b, b'} = \E\left(\nu(\cdot, R(b) | B(b')) \mid B(b')\right)$.

\end{lemma}
\begin{proof}
Let $b, b' \in \{0, 1\}$ be arbitrary. For any outcome $\{B(b') = z\}$, let $\P_z(A(x_b) \in \cdot)$ be the probability measure $\P(A(x_b) \in \cdot | B(b') = z)$. By the assumptions of conditional differential privacy~\eqref{def:cdp}, it follows that under the probability measure $\P_z$, $A(x_b)$ is $(\epsilon(z), \delta(z))$-differentially private.  Moreover, it also follows that $R$ is an instance of $(\epsilon(z), \delta(z))$-randomized response under $\P_z$. Consequently, Lemma~\ref{fact:post_proc_rr} yields the existence of a kernel $\nu_z$ such that $\P_z(A(x_b) \in \cdot) = \E \nu_z(\cdot, R(b))$. Setting $\nu(\cdot, R(b) | z) := \nu_{z}(\cdot, R(b))$ thus yields the desired result.
\end{proof}


%A proof of the above lemma can be found in the appendix. 
We now explain heuristically how Lemma~\ref{lem:cond_post_rr} will allow us to prove Theorem~\ref{thm:fully_adaptive}. At a high-level, for any fixed $x \in \calX$ and neighbor $x' \sim x$, we will reduce the study of the composition of arbitrary conditionally differentially private algorithms to that of conditional randomized response, where we are conditioning always on the natural filtration generated by the outputs of the algorithms. Since conditional randomized response is probabilistically differentially private, we can appeal to Theorem~\ref{thm:new_filter} to show that the composition of the conditional randomized-response algorithms is $(\epsilon, \delta)$-pDP, and hence by Lemma~\ref{lem:dp_to_pdp} also $(\epsilon, \delta)$-DP. Lastly, we use Lemma~\ref{lem:cond_post_rr} alongside the fact that differential privacy is closed under arbitrary randomized post-processing \cite{dwork2014algorithmic} to prove the result.

%We now formalize the above heuristic argument in the following proof.

\begin{proof}[\textbf{Proof of Theorem~\ref{thm:fully_adaptive}}]
Fix an arbitrary input dataset $x_0 \in \calX$ and neighboring dataset $x_1 \in \calX$. Let $(R_n)_{n \geq 1}$ be a sequence of algorithms such that $R_n$ is an instance of $(\epsilon_n, \delta_n)$-randomized response conditioned on the randomized algorithm $(A_{1:n - 1}(x_{(\cdot)}), B_{1: n - 1}(x_{(\cdot)})) : \{0, 1\} \rightarrow \calY^{n - 1} \times \calZ^{n - 1}$ (where the notation $x_{(\cdot)}$ is as outlined in Lemma~\ref{lem:cond_post_rr}).

Lemma~\ref{lem:cond_post_rr} guarantees the existence of a sequence of transition kernels $(\nu_n)_{n \geq 1}$ such that, for all $n \geq 1$ and $b, b' \in \{0, 1\}$, we have $\P(A_n(x_b) \in \cdot \mid A_{1:n - 1}(x_{b'}), B_{1:n - 1}(x_{b'})) = \nu^{(n)}_{b, b'}$ almost surely, where $\nu^{(n)}_{b, b'}$ is defined in terms of $\nu_n$ as in the lemma statement. In particular, it follows that, for any $n \geq 1$, $\P(A_{1:n}(x_b) \in \cdot ) = \nu^{(1)}_{b, b'} \otimes \cdots \otimes \nu^{(n)}_{b, b'}$, where $\mu \otimes \rho$ indicates the product measure between $\mu$ and $\rho$. 

Now, for any $n \geq 1$, since $R_n$ is an instance of $(\epsilon_n, \delta_n)$-randomized response conditioned on $(A_{1:n - 1}, B_{1: n - 1})$, it follows that $R_n$ is in fact $(\epsilon_n, \delta_n)$-pDP conditioned on $(A_{1:n - 1}, B_{1: n - 1})$. Moreover, this also implies that $R_n$ is $(\epsilon_n, \delta_n)$-pDP conditioned on $(A_{1:n - 1}, B_{1:n - 1}, R_{1:n - 1})$, since by assumption $\epsilon_n$ and $\delta_n$ are just deterministic functions of the random outputs of $A_{1:n - 1}$ and $B_{1: n -1}$. Thus, by Theorem~\ref{thm:new_filter}, it follows that $R_{1:N(x_{(\cdot)})}(\cdot)$ is $(\epsilon, \delta)$-pDP, where $\epsilon, \delta$ and $N$ are as outlined in the statement of Theorem~\ref{thm:fully_adaptive} and the notation $N(x_{(\cdot)})$ indicates that $N$ is a function of $x_b$, for $b \in \{0, 1\}$. 

Now, by Lemma~\ref{lem:dp_to_pdp}, it follows that $R_{1 : N(x_{(\cdot)})}(\cdot)$ is also $(\epsilon, \delta)$-differentially private. Since differential privacy is closed under arbitrary randomized post-processing \cite{dwork2014algorithmic}, and since for any $n \geq 1$ $A_{1:n}(x_b)$ has law $\nu_{b, b'}^{(1)} \otimes \cdots \otimes \nu^{(n)}_{b, b'}$, it follows that $A_{1:N(\cdot)}(\cdot)$ is $(\epsilon, \delta)$-differentially private as well, proving the desired result.
\end{proof}

Lastly, as in the end of Section~\ref{sec:filter} in Theorem~\ref{thm:zcdp},  we can extend Theorem~\ref{thm:fully_adaptive} to include the case where some of the algorithms instead satisfy conditional zero-concentrated differential privacy instead of conditional differential privacy. As before, we relegate the proof of the theorem to Appendix~\ref{app:zcdp}.

\begin{comment}
We again omit the proof, as the result follows from only reducing the algorithms that satisfy conditional differential privacy to instances of conditional randomized response. As mentioned in the justification preceding Corollary~\ref{cor:zcdp}, algorithms satisfying zero-concentrated differential privacy already satisfy a subGaussian-like characterization of privacy loss, and hence do not need to be touched.
\end{comment}
\begin{theorem}
\label{thm:zcdp_fully}
Let $(A_n)_{n \geq 1}$ and $(B_n)_{n \geq 1}$ be algorithms as mentioned in the statement of Theorem~\ref{thm:fully_adaptive}, and for any $n$ and $x$ let $\calF_n(x) := \sigma\left(A_m(x), B_m(x) : m \leq n \right)$. For any $n \geq 1$, assume there are functions $\epsilon_n, \delta_n : \calY^{n - 1} \times \calZ^{n - 1} \rightarrow \R_{\geq 0}$. For any $x \sim x'$ neighbors, assume that with probability 1 we have either
\begin{enumerate}
    \item $\P(A_{1:n}(x) \in G \mid \calF_{n - 1}(x)) \leq e^{\epsilon(x)}\P(A_{1:n}(x') \in G \mid \calF_{n - 1}(x)) + \delta(x)$ for all $G \in \calG$, or
    \item $\delta_n(x) = 0$ and $\E\left(e^{\lambda \calL_n(x, x')} \mid \calF_{n - 1}(x)\right) \leq e^{\frac{1}{2}\lambda(\lambda + 1)\epsilon_n(x)^2}$ for all $\lambda \geq 0$.
\end{enumerate}
Then, for any $\epsilon >0$ and $\delta = \delta' + \delta''$, letting $N$ be as outlined in Theorem~\ref{thm:fully_adaptive}, we have that the algorithm $A_{1:N(\cdot)}(\cdot)$ is $(\epsilon, \delta)$-differentially private.
\end{theorem}

==> Old_Tex/FullyAdaptiveOLD.tex <==
\section{Fully Adaptive Composition}
\label{sec:fully_adaptive}

In the previous section, we demonstrated how to match the composition rate of advanced composition under the assumption that the algorithms beings composed satisfy condition probabilistic differential privacy. As noted in Lemma~\ref{lem:dp_to_pdp}, there is in fact a gap between probabilistic differential privacy and (standard) differential privacy: all algorithms that satisfy probabilistic differential privacy also satisfy differential privacy, but the converse is not true. Thus, in order to prove our results in Section~\ref{sec:filter}, we needed to place stronger assumptions on the algorithms being composed than desired. In this section, we demonstrate our results in Section~\ref{sec:filter} actually still do essentially hold under the weaker assumption that the algorithms being composed satisfy conditional differential privacy.

In short, our goal in this section is to prove the following theorem.

\begin{theorem}
\label{thm:fully_adaptive}
Suppose $(A_n)_{n \in \N}$ is a sequence of algorithms, $\{(\calF_n(x))_{n \in \N}\}_{x \in \calX}$ a collection of filtrations, and $\{(\epsilon_n(x), \delta_n(x))_{n \in \N}\}_{x \in \calX}$ a collection of privacy parameters such that $A_n$ is $(\epsilon_n, \delta_n)$-DP conditioned on $\calF_{n - 1}$, for all $n \in \N$. Let $\epsilon > 0$ be a target privacy parameter, and $\delta = \delta' + \delta''$ a target approximation parameter such that $\delta' > 0, \delta'' \geq 0$. For any $x \in \calX$, define the $(\calF_n(x))_{n \in \N}$-stopping time $N(x)$ by
$$
N(x) := \inf\left\{n \in \N : \epsilon < \sqrt{2\log\left(\frac{1}{\delta'}\right)\sum_{m \leq n + 1}\epsilon_m(x)^2} + \frac{1}{2}\sum_{m \leq n + 1}\epsilon_m(x)^2\right\} \wedge \inf\left\{n \in \N : \delta'' <  \sum_{m \leq n + 1}\delta_m(x)\right\},
$$
where $a \land b := \min\{a, b\}$. Then, the algorithm $A_{1:N(\cdot)}(\cdot) : \calX \rightarrow \calY^\infty$ is $(\epsilon, \delta)$-differentially private.
\end{theorem}

The statement of Theorem~\ref{thm:fully_adaptive} appears essentially the same as Theorem~\ref{thm:new_filter}. However, there are two differences. First, as mentioned in the previous paragraph, we loosen the assumption of conditional probabilistic differential privacy to that of just conditional differential privacy. Secondly, we claim that the composed algorithm is $(\epsilon, \delta)$-differentially private. In particular, we make no claims about the privacy loss of the composed interaction. This is because, in general, probabilistic differential privacy and differential privacy are \textit{not} equivalent, per Lemma~\ref{lem:dp_to_pdp}. 

It turns out that in order to prove Theorem~\ref{thm:fully_adaptive}, we need some additional machinery. In particular, we need to briefly study and generalize what is perhaps the simplest example of a differentially private algorithm: randomized response. The setup for randomized response is simple. The space of datasets is simply $\{0, 1\}$, i.e. a dataset consists of a single hidden bit. The mechanism works by keeping the hidden bit the same with some probability, and flipping the bit with some comparable but smaller probability. Lastly, with some small probability, the true underlying dataset is revealed. Formally, randomized response is defined as follows.

\begin{definition}
\label{def:rr}
Let $\calR := \{0, 1, \top, \bot\}$ and $2^\calR$ the corresponding power set of $\calR$. Then, the pair of random variables $\{R(b)\}_{b \in \{0, 1\}}$ defined on a common probability space $(\Omega, \calF, \P)$ and taking values in the measurable space $(\calR, 2^\calR)$ is set to be an instance of $(\epsilon, \delta)$-randomized response if $R(b)$ has the following distribution.
$$
R(b) = \begin{cases} b \qquad \text{with probability } (1 - \delta)\frac{e^\epsilon}{1 + e^\epsilon} \\
1 - b \qquad \text{with probability } (1 - \delta)\frac{1}{1 + e^\epsilon}\\
\top \qquad \text{with probability } \delta \text{ if } b = 1\\
\bot \qquad \text{with probability } \delta \text{ if } b = 0.
\end{cases}
$$
\end{definition}

It can unsurprisingly be checked that $(\epsilon, \delta)$-randomized response, as outlined above, is in fact $(\epsilon, \delta)$-DP. In addition, $(\epsilon, \delta)$-randomized response also satisfies the guarantees of probabilistic differential privacy. What is surprising, however, is that \textit{any} $(\epsilon, \delta)$-DP algorithm can actually viewed as a randomized post-processing of randomized response \cite{kairouz2015composition} \cite{murtagh2016complexity}. In particular, the following technical fact is true.

\begin{fact}
\label{fact:post_proc_rr}
Let $A$ be a $(\epsilon, \delta)$-differentially private algorithm defined on some probability space taking datasets in $\calX$ to outputs in the measurable space $(\calY, \calG)$. Let $\{R(b)\}_{b \in \{0, 1\}}$ be an instance of $(\epsilon, \delta)$-randomized response defined on a probability space $(\Omega, \calF, \P)$. Then, for any input dataset $x \in \calX$ and any neighboring dataset $x' \sim x \in \calX$, there is a random function $f_{x, x'} : \Omega \times \calR \rightarrow \calY$ such that
\begin{enumerate}
\item $f_{x, x'}$ is independent of $\{R(b)\}_{b \in \{0, 1\}}$, 
\item $f_{x, x'}(R(0)) =_{d} A(x)$, and
\item $f_{x, x'}(R(1)) =_{d} A(x')$.
\end{enumerate}

\end{fact}


Fact~\ref{fact:post_proc_rr} is a very powerful result --- in fact it can be used to prove advanced composition \arcomment{\cite{}}. However, we need a slightly more detailed result to hold. This is because we want to allow privacy parameters to be adaptively selected over time. To facilitate a generalization, we first describe a generalization of randomized response to a conditional setting --- that is a setting wherein the parameters $\epsilon$ and $\delta$ associated with randomized response can be selected according to some auxiliary information. We define conditional randomized response as follows.

\begin{definition}
\label{def:cond_rr}
Let $\calR := \{0, 1, \top, \bot\}$ and $2^\calR$ the corresponding power set of $\calR$. Let $\{R(b)\}_{b \in \{0, 1\}}$ be a pair of random variables defined on a common probability space $(\Omega, \calF, \P)$ and taking values in the measurable space $(\calR, 2^\calR)$. Let $\calH \subset \calF$ be a sub $\sigma$-algebra. Then, $\{R(b)\}_{b \in \{0, 1\}}$ is said to be an instance of $(\epsilon, \delta)$-randomized response conditioned on $\calH$ if the following hold:
\begin{enumerate}
    \item $\epsilon, \delta$ are non-negative $\calH$-measurable random variables, and
    \item For any $b \in \{0, 1\}$ and any $\omega \in \Omega$, the conditional probability $\P(R(b) \in \cdot | \calH)(\omega) : 2^\calR \rightarrow [0, 1]$ is equal to the law of $(\epsilon_n(\omega), \delta_n(\omega))$-randomized response with input $b$.
\end{enumerate}

\end{definition}

Definition~\ref{def:cond_rr}, heuristically, tells us that once we observe the information available in $\calH$, the conditional laws of $R(0)$ and $R(1)$ just become that of regular randomized response with some known privacy parameters. Suppose there are two sub $\sigma$-algebras $\calH(0), \calH(1) \subset \calF$ and random privacy parameter pairs $\{(\epsilon(b), \delta(b))\}_{b \in \{0, 1\}}$  such that $R$ is an instance $(\epsilon(b), \delta(b))$-randomized response conditioned on $\calH(b)$, for all $b \in \{0, 1\}$. In this case, it is immediate to see that $R$ is both $(\epsilon, \delta)$-differentially private conditioned on $\calH$ and $(\epsilon, \delta)$-pDP conditioned on $\calH$. Using the above generalization of randomized response, we can formulate a conditional analogue of Fact~\ref{fact:post_proc_rr}. 

\begin{lemma}
\label{lem:cond_post_rr}
Let $A$ be an algorithm taking inputs in $\calX$ to outputs in a measurable space $(\calY, \calG)$, $\{(\epsilon(x), \delta(x))\}_{x \in \calX}$ a collection of (random) privacy parameters, and $\{\calH(x) \}_{x \in \calX}$ a collection of $\sigma$-algebras. Suppose $A$ is $(\epsilon, \delta)$-differentially private conditioned on $\calH$. Fix an input $x \in \calX$, and suppose $\{R(b)\}_{b \in \{0, 1\}}$ are random variables defined on the same probability space as  $\{A(x)\}_{x \in \calX}$, and that $R$ is an instance of $(\epsilon, \delta)$-randomized response given $\calH(x)$. Then, for any neighbor $x' \sim x \in \calX$, there is a random function $f_{x, x'} : \Omega \times \calR \rightarrow \calY$ such that
\begin{enumerate}
    \item $f_{x, x'}(\cdot, r)$ is independent of $\{R(b)\}_{b \in \{0, 1\}}$, for all $r \in \calR$,
    \item $\P\left(f_{x, x'}(R(0)) \in G | \calH(x)\right) = \P\left(A(x) \in G | \calH(x)\right)$, for all $G \in \calG$, and
    \item $\P\left(f_{x, x'}(R(1)) \in G | \calH(x)\right) = \P\left(A(x') \in G | \calH(x)\right)$.
\end{enumerate}


\end{lemma}

%A proof of the above lemma can be found in the appendix. 
We now explain heuristically how Lemma~\ref{lem:cond_post_rr} will allow us to prove Theorem~\ref{thm:fully_adaptive}. At a high-level, for any fixed $x \in \calX$, we will reduce the study of the composition of arbitrary conditionally differentially private algorithms to that of conditional randomized response, where we are conditioning always on the natural filtration generated by the outputs of the algorithms. Since conditional randomized response is probabilistically differentially private, we can appeal to Theorem~\ref{thm:new_filter} to show that the composition of the conditional randomized-response algorithms is $(\epsilon, \delta)$-pDP, and hence by Lemma~\ref{lem:dp_to_pdp} also $(\epsilon, \delta)$-DP. Lastly, we use Lemma~\ref{lem:cond_post_rr} alongside the fact that differential privacy is closed under arbitrary post-processing to prove the result.

%We now formalize the above heuristic argument in the following proof.

\begin{comment}
\begin{proof}[\textbf{Proof of Theorem~\ref{thm:fully_adaptive}}]
Fix $x \in \calX$ and a neighboring dataset $x' \in \calX$.  Let $\{(R_n(b))_{n \in \N}\}_{b \in \{0, 1\}}$ such that, for all $n \in \N$, $R_n$ is an instance of $(\epsilon_n(x_b), \delta_n(x_b))$-randomized response conditioned on $\calF_{n - 1}(x_b)$, for all $b \in \{0, 1\}$, where $x_b = x$ if $b = 0$ and $x_b = x'$ if $b = 1$. Then, for all $n \in \N$, Lemma~\ref{lem:cond_post_rr} yields the existence of random function $f^{(n)}_{x, x'}$ such that the law of $f^{(n)}_{x, x'}(R_n(b))$ conditioned on $\calF_{n - 1}(x)$ is equal to the law of $A_n(x_b)$ conditioned on $\calF_{n - 1}(x)$. In particular, since all the conditional distributions are the same, it follows that $(f^{(1)}_{x, x'}(R_1(b)), \dots, f^{(n)}_{x, x'}(R_n(b))) =_d A_{1:n}(x_b)$, for all $n \in \N$ and $b \in \{0, 1\}$, and consequently also that $(f^{(1)}(R_1(b)), \dots, f^{(N(x))}_{x, x'}(R_{N(x)}(b))) =_d A_{1:N(x)}(x_b)$, for all $b \in \{0, 1\}$.

Now, since $\{R_n(b)\}_{b \in \{0 ,1\}}$ is $\{(\epsilon_n(x_b), \delta_n(x_b))\}_{b \in \{0, 1\}}$-probabilistically differentially private conditioned on $\{\calF_{n - 1}(x_b)\}_{b \in \{0, 1\}}$, Theorem~\ref{thm:new_filter} yields that the composed algorithm $R_{1:N(\cdot)}(\cdot)$ is $(\epsilon, \delta)$-probabilistically differentially private. Thus, by Lemma~\ref{lem:dp_to_pdp}, it follows that $R_{1:N(\cdot)}(\cdot)$ is $(\epsilon, \delta)$-differentially private as well. Defining the randomized post-processing function $F_{x, x'}$ by $F_{x, x'}(R_{1:N(x_b)}(b)) = (f^{(1)}_{x, x'}(R_1(b)), \dots, f^{N(x)}_{x, x'}(R_{N(x_b)}(b)))$, by closure under post-processing, it follows that $F_{x, x'} \circ R_{1:N(\cdot)}(\cdot)$ is $(\epsilon, \delta)$-differentially private. Consequently, letting $G$ be an arbitrary measurable set of outcomes, we have that, for all $b \in \{0, 1\}$,
$$
\P(A_{1:N(x_b)}(x_b) \in G) = \P(F_{x, x'}(R_{1:N(x_b)}(b)) \in G) \leq e^\epsilon \P(F_{x, x'}(R_{1:N(x_{1 - b})}(1 - b)) \in G) + \delta = \P(A_{1:N(x_{1 - b})}(x_{1 - b}) \in G).
$$

Since $x, x' \in \calX$ were arbitrary neighboring datasets, the result follows.
\end{proof}
\end{comment}

==> Old_Tex/MartingalesOLD.tex <==
\section{Privacy Loss Martingales and Time-uniform Concentration}
\label{sec:martingales}

\subsection{Martingales and Concentration Preliminaries}
\label{sec:martingales:basics}
Now the we have introduced a measure-theoretic framework for studying differential privacy and privacy loss, we can discuss a useful tool for proving privacy loss composition results: privacy loss martingales. Before going forward, we briefly define the measure-theoretic notions of martingales and supermartingales, as these will be essential in the sequel.

We start with an intuitive definition. A discrete time stochastic process is a martingale if, given all available information up to and including time $n - 1$, our best guess for where the process will be at time $n$ is where the process is at time $n - 1$. More formally, we can define martingales as follows.

\begin{definition}
\label{def:mart}
Suppose we are given a filtration $(\calF_n)_{n \in \N}$ of a $\sigma$-algebra $\calF$ and stochastic process $(X_n)_{n \in \N}$ defined on a probability space $(\Omega, \calF, \P)$. Then, we say that an  process $(X_n)_{n \in \N}$ is a \textit{martingale} with respect to $(\calF_n)_{n \in \N}$ if (a) $(X_n)_{n \in \N}$ is adapted to $(\calF_n)_{n \in \N}$, i.e. $X_n$ is $\calF_n$-measurable, for all $n \in \N$, (b) $\E|X_n| <\infty$ for all $n \in \N$, i.e. the process $(X_n)_{n \in \N}$ is integrable, and (c) $\E(X_n | \calF_{n - 1}) = X_{n - 1}$, for all $n \geq 1$.
% \end{enumerate}

We say that $(X_n)_{n \in \N}$ is a \textit{supermartingale} with respect to $(\calF_n)_{n \in \N}$ the third condition is replaced with $\E(X_n | \calF_{n - 1}) \leq X_{n - 1}$, for all $n \geq 1$. That is, a supermartingale is a process which tends not to increase.
\end{definition}

Definition~\ref{def:mart} exactly formalizes the aforementioned intuition. Note that every martingale is also a supermartingale, but not every supermartingale is a martingale. Martingales are useful because they offer very strong, time-uniform concentration of measure properties, as will be seen shortly. These concentration properties will allow us to prove strong composition results for private algorithms based on the privacy parameters witnessed. 

At the heart of martingale concentration is Ville's inequality~\cite{ville1939etude, howard2020line}, which provides time-uniform upper bounds on nonnegative supermartingales. 
% In particular, Ville's inequality tells us the following:

\begin{fact}[\textbf{Ville's Inequality}]
\label{fact:ville}
Let $(X_n)_{n \in \N}$ be a nonnegative supermartingale with respect to some filtration $(\calF_n)_{n \in \N}$. Then, for any confidence parameter $\delta \in (0, 1)$, we have 
\(
\P\left(\exists n \in \N : X_n \geq \frac{\E X_0}{\delta}\right) \leq \delta.
\)

\end{fact}

We do not directly leverage Ville's inequality in this work, but all inequalities we use can be directly proven from Fact~\ref{fact:ville}. In particular, to obtain the privacy composition same rates as advanced composition, we need the following recent advance in time-uniform martingale concentration~\cite{howard2020line}.

\begin{fact}
\label{fact:line_cross}
Let $(M_n)_{n \in \N}$ be a martingale with respect to some filtration $(\calF_n)_{n \in \N}$ such that $M_0 = 0$ almost surely. Moreover, let $(\sigma_n)_{n \in \N}$ be a $(\calF_n)_{n \in \N}$-predictbale sequence of random variables such that, conditioned on $\calF_{n - 1}$, $\Delta M_n := M_n - M_{n - 1}$ is $\sigma_n^2$-subGaussian.
Define $V_n := \sum_{m \leq n}\sigma_m^2$. Then, we have, for all $a, b > 0$, 
$$
\P\left(\exists n \in \N : M_n \geq \frac{b}{2} + \frac{b}{2a}V_n\right) \leq \exp\left(\frac{-b^2}{2a}\right).
$$

\end{fact}

The predictable process $(V_n)_{n \in \N}$ is a proxy for the accumulated variance of $(M_n)_{n \in \N}$ up to any fixed point in time. In particular, the process $(V_n)_{n \in \N}$ can be thought of as yielding the \textit{intrinsic time} of the process. The free parameters $a$ and $b$ thus allow us to optimize the tightness of the boundary for some intrinsic moment in time. This is ideal for us, as, for the sake of composition, the target privacy parameter $\epsilon$ can guide us in finding a point in intrinsic time (that is, in terms of the process $(V_n)_{n \in \N}$) to optimize for. We discuss how to apply this inequality to prove privacy composition results in Section~\ref{sec:filter}.

We also leverage the following martingale inequalities from \cite{howard2021unif} in Section~\ref{sec:odometers}, where we construct various families of time-uniform bounds on privacy loss in fully-adaptive composition. These inequalities take on a more complicated form than Fact~\ref{fact:line_cross}, but we explain the intuition behind them in the sequel. The first bound we present relies on the method of mixtures for martingale concentration. A good background on this technique can be found in \cite{kaufmann2018mixture}, \cite{delapena2007maximization}, and \cite{howard2021unif}.

\begin{fact}
\label{fact:mixture}
Let $(M_n)_{n \in \N}$ be a martingale with respect to some filtration $(\calF_n)_{n \in \N}$ such that $M_0 = 0$ almost surely. Moreover, let $(\sigma_n)_{n \in \N}$ be a $(\calF_n)_{n \in \N}$-predictbale sequence of random variables such that, conditioned on $\calF_{n - 1}$, both $\Delta M_n := M_n - M_{n - 1}$ and $-\Delta M_n$ are $\sigma_n^2$-subGaussian.
Define $V_n := \sum_{m \leq n}\sigma_m^2$. Then, for any $\rho > 0$, for any $\delta > 0$ we have
$$
\P\left(\exists n \in \N : M_n \geq \sqrt{2(V_n + \rho)\log\left(\frac{1}{\delta}\sqrt{\frac{V_n + \rho}{\rho}}\right)}\right) \leq \delta.
$$

\end{fact}

The next inequality relies on the recent technique of boundary stitching, first presented in \cite{howard2021unif}. Intuitively, the technique works by breaking intrinsic time (that is, time according to the accumulated variance process $(V_n)_{n \in \N}$) into roughly geometrically spaced pieces. Then, one optimizes a tight-boundary in said region and takes a union bound. The actual details are more technical, but are not needed in this work. 

\begin{fact}
\label{fact:stitch}
Let $(M_n)_{n \in \N}$ be a martingale with respect to some filtration $(\calF_n)_{n \in \N}$ such that $M_0 = 0$ almost surely. Moreover, let $(\sigma_n)_{n \in \N}$ be a $(\calF_n)_{n \in \N}$-predictbale sequence of random variables such that, conditioned on $\calF_{n - 1}$, both $\Delta M_n := M_n - M_{n - 1}$ and $-\Delta M_n$ are $\sigma_n^2$-subGaussian.
Define $V_n := \sum_{m \leq n}\sigma_m^2$. Then, for any fixed $v_0 > 0$ and confidence parameter $\delta \in (0, 1)$, we have
$$
\P\left(\exists n \in \N : M_n \geq 1.7\sqrt{V_n\left(\log\log\left(\frac{2V_n}{v_0}\right) + 0.72\log\left(\frac{5.2}{\delta}\right)\right)}, \; V_n \geq v_0\right) \leq \delta.
$$

\end{fact}

Note that the original version of Fact~\ref{fact:stitch} as found in \cite{howard2021unif} had more free parameters to optimize over, but we have already simplified the expression to make the Fact more readable. The free parameter $v_0 > 0$ in the above boundary gives the intrinsic time at which the boundary becomes non-trivial (i.e., the tightest available upper bound before $V_n \geq v_0$ is $\infty$). 

We hold off on qualitatively comparing these bounds until Section~\ref{sec:odometers:comparison}, where we construct various time-uniform bounds on privacy loss processes. For now, Fact~\ref{fact:line_cross} can be thought of as providing a tight upper bound on a martingale at a single point in intrinsic time, providing loose guarantees elsewhere. On the other hand, Facts~\ref{fact:mixture} and \ref{fact:stitch} provide decently tight control over a martingale at all points in intrinsic time simultaneously, although sacrificing tightness at any given fixed point in intrinsic time.

Lastly, let $(U_n)_{n \in \N}$ be any of the upper bounds on $(M_n)_{n \in \N}$ discussed in Facts~\ref{fact:line_cross}, \ref{fact:mixture}, and \ref{fact:stitch}. By the guarantees above, we have $\P(\exists n \in \N: M_n > U_n) \leq \delta$. Consequently, due to the time-uniform nature of these bounds, if $N$ is a $(\calF_n)_{n \in \N}$ stopping time (or, even more generally, just a random time), we in fact get the guarantee that $\P(M_N > U_N) \leq \delta$. This validity of bounds at stopping times is what will allow us to prove our composition results in the upcoming sections.



\subsection{Privacy Loss Martingales}
\label{sec:martingales:ploss}
Our goal in this paper, as illustrated in the introduction, is twofold. First, we want to match the tightness of advanced composition while allowing both privacy parameters and algorithms to be chosen adaptively. Second, we want to provide strong, time-uniform bounds on privacy loss for setting where target privacy levels or stopping conditions may not be known in advance.

To address these goals, we adopt the privacy composition terminology as introduced in \cite{rogers2016odometer}. In particular, the authors introduce two probabilistic objects to address the problem of fully-adaptive composition. One object, called a \textit{privacy filter}, is a stopping time $N$ that guarantees, if we stop at time $N$, the total composed interaction will be differentially private with preset target parameters. The other object, called a \textit{privacy odometer}, aims to provide a time-uniform upper bound on the accumulated privacy loss. We now define these objects in our framework for conditional differential privacy.

\begin{definition}
\label{def:filter}
Let $(A_n)_{n \in \N}$ be an adaptively chosen sequence of algorithms and $\{(\calF_n(x))_{n \in \N}\}_{x \in \calX}$ a collection of filtrations such that $A_n$ is $(\epsilon_n, \delta_n)$-pDP conditioned on $\calF_{n - 1}$. Let $\epsilon > 0$ be a target privacy parameter and $\delta > 0$ a target approximation parameter. Then, a collection of random times $\{N(x)\}_{x \in \calX}$ such that $N(x)$ is a $(\calF_n(x))_{n \in \N}$-stopping time is an  \textit{$(\epsilon, \delta)$-privacy filter} if the algorithm $A_{1:N(\cdot)}(\cdot)$ is $(\epsilon, \delta)$-pDP.
\end{definition}

What Definition~\ref{def:filter} tells us is that, essentially, a privacy filter is just a condition for determining whether or not to stop composing algorithms based on the observed algorithm outputs. However, in all of our considerations, the stopping time will only depend on the outputs of the algorithms through the corresponding privacy parameters (recall that, by the assumption of conditional $(\epsilon_n, \delta_n)$-pDP, $\epsilon_n(x)$ and $\delta_n(x)$ are predictable with respect to $(\calF_n(x))_{n \in \N}$, for all $n \in \N$).

We can also correspondingly define privacy odometers.

\begin{definition}
\label{def:odometer}
Let $(A_n)_{n \in \N}$ be an adaptively chosen sequence of algorithms and $\{(\calF_n(x))_{n \in \N}\}_{x \in \calX}$ a collection of filtrations such that $A_n$ is $(\epsilon_n, \delta_n)$-pDP conditioned on $\calF_{n - 1}$. Let $\delta \in (0, 1)$ be a target confidence paramter. Then, a collection of sequences of random variables $\{(U_n(x))_{n \in \N}\}_{x \in \calX}$ is a $\delta$-privacy odometer if 
\begin{enumerate}
    \item $(U_n(x))_{n \in \N}$ is $(\calF_n(x))_{n \in \N}$-predictable, for all $x \in \calX$, and
    \item For any input database $x \in \calX$ and any neighbor $x'\sim x\in \calX$, we have
    $$
    \P\left(\exists n \in \N : \calL_{1:n}(x, x') > U_n(x)\right) \leq \delta.
    $$
\end{enumerate}
\end{definition}

Once again, as with many definitions seen throughout this paper, we need to define a separate random sequence for each $x \in \calX$ because the sequence of upper bounds constituting the odometer ultimately will depend on the underlying dataset (even if only by proxy of the released predictable streams of privacy parameters).

To construct these objects, the authors in \cite{rogers2016odometer} rely on self-normalized concentration inequalities -- for instance those found in \cite{de2004self} and \cite{chen2014exponential}. However, given the background on time-uniform concentration presented in the previous subsection, we instead opt to use these time-uniform bounds to construct our improved filters and odometers. Before we can apply the bounds to construct these objects, we must use the privacy loss processes associated with algorithm composition to construct a martingale. 

As such, for the final part of our background, we introduce what are known in the literature as \textit{privacy loss martingales}. These martingales have been used to prove a plethora of well-known privacy composition results \cite{dwork2014algorithmic} \cite{bun2016concentrated}. Going forward, we fix a family of filtrations $\{(\calF_n(x))_{n \in \N}\}_{x \in \calX}$. To simplify our presentation of privacy loss martingales, we assume the algorithms $(A_n)_{n \in \N}$ are all $(\epsilon_n, 0)$ -pDP with respect to $\calF_{n - 1}$. We discuss how to handle the more general case of $\delta_n > 0$ in subsequent sections. For any fixed $x \in \calX$ and neighboring dataset $x' \sim x \in \calX$, it is clear that the process $(M_n)_{n \in \N}$ defined as
$$
M_n := M_n(x, x') := \calL_{1:n}(x, x') - \sum_{m \leq n}\E\left(\calL_{m}(x, x')| \calF_{n - 1}(x)\right)
$$
is a martingale with initial value 0 with respect to $(\calF_n(x))_{n \in \N}$. This process is what we call the privacy loss martingale associated with databases $x, x' \in \calX$. Moreover, we can define the \textit{increments} of $(M_n)_{n \in \N}$ as the process $(\Delta M_n)_{n \in \N}$ given by
$$
\Delta M_n := M_n - M_{n - 1} = \calL_n(x, x') - \E\left(\calL_n(x, x')|\calF_{n - 1}(x)\right).
$$
By the assumption of conditional $(\epsilon_n, 0)$-pDP, it is immediate that, for all $n \in \N$, $\Delta M_n$ and $-\Delta M_n$ are $\epsilon_n^2$-subGaussian. Thus, we will directly be able to apply the various time-uniform bounds to the problems at hand. Without further ado, we now proceed to our presentation of our improved fully-adaptive composition results.

==> Old_Tex/OdometersOLD.tex <==
\section{Time Uniform Privacy Loss Bounds}
\label{sec:odometers}
In Sections~\ref{sec:filter} and \ref{sec:fully_adaptive}, we showed that one could obtain the same composition rate as advanced composition while being able to adaptively select \textit{both} the algorithms and privacy parameters being used. The catch was that the total level of privacy (determined by global parameters $\epsilon, \delta \geq 0$) must be fixed in advance. For practitioners aiming to obtain differential privacy guarantees, such a prefixed level is unavoidable. However, in many modern, machine learning settings, privacy may be a secondary concern to objectives such as accuracy or utility \cite{ligett2017accuracy} \cite{whitehouse2021noise}. Thus, it is desirable to have tight control over accumulated privacy loss not just at the stopping times constructed in Theorem~\ref{thm:new_filter}, but at all stopping times simultaneously.

In this section, our goal is to provide general classes of time-uniform high-probability bounds on the privacy loss of composed interactions. In particular, going forward, we adopt the terminology of \cite{rogers2016odometer} and call such bounds \textit{privacy odometers}, as in Definition~\ref{def:odometer}. While in Section~\ref{sec:fully_adaptive} we were able to make the assumption that the algorithms being composed were conditionally differentially private, here, we need to settle for the stronger assumption of conditional probabilistic privacy. This is because our goal is not overall differential privacy, but rather tight control directly over the privacy loss processes.

Our main point of comparison in this section is the following original privacy odometer~\cite{rogers2016odometer}.

\begin{fact}[\textbf{Theorem 6.5 in \cite{rogers2016odometer}}]
\label{fact:rogers_odometers}
Let $(A_n)_{n \in \N}$ be a sequence of algorithms taking inputs in some space $\calX$ to outputs in some measurable space $(\calY, \calG)$. Let $\{(\calF_n(x))_{n \in \N}\}_{x \in \calX}$ be a collection of filtrations and $\{(\epsilon_n(x), \delta_n(x))_{n \in \N}\}_{x \in \calX}$ a collection of sequences of privacy parameters. Assume that $A_n$ is $(\epsilon_n, \delta_n)$-pDP conditioned on $\calF_{n - 1}$.  Fix $\delta = \delta' + \delta''$, where $\frac{1}{e} \geq \delta' > 0$ and $\delta'' \geq 0$.  For any $x \in \calX$, define the stopping time
$$
N(x) := \inf\left\{n \in \N : \delta'' < \sum_{m \leq n +1}\delta_m(x)\right\},
$$
where $|x|$ denotes the number of elements in dataset $x$. Define the random sequences $(W_n(x))_{n \in \N}$ and $(V_n(x))_{n \in \N}$ by
\begin{align*}
W_n(x) &:= \sqrt{2\sum_{m \leq n}\epsilon_m(x)^2\left( \log(110e) + 2\log\left(\frac{\log(|x|)}{\delta'}\right)\right)} + \frac{1}{2}\sum_{m \leq n}\epsilon_m(x)(e^{\epsilon_m(x)} - 1),\\
V_n(x) &:= \sqrt{2\left(\frac{1}{|x|^2} + \sum_{m \leq n}\epsilon_m(x)^2\right)\left(1 + \frac{1}{2}\log\left(1 + |x|^2\sum_{m \leq n}\epsilon_m(x)^2\right)\right)\log\log\left(\frac{4}{\delta'}\log_2(|x|)\right)}.
\end{align*}
Then, the collection of sequences $\{(U^{\mathrm{R}}(x)_n)_{n \in \N}\}_{x \in \calX}$ given by
$$
U_n^{\mathrm{R}}(x) := \left(W_n(x)\one_{\sum_{m \leq n}\epsilon_m(x)^2 \in \left[\frac{1}{|x|^2}, 1\right]} + V_n(x)\one_{\sum_{m \leq n}\epsilon_m(x)^2 \notin \left[\frac{1}{|x|^2}, 1\right]}\right)\one_{n \leq N(x)} + \infty\one_{n > N(x)}
$$
is a $\delta$-privacy odometer.


\end{fact}

The odometer presented above in Fact~\ref{fact:rogers_odometers} suffers from a variety of downsides. To start, the odometer has an explicit dependence on the size of the underlying dataset, denoted as $|x|$. Since, in many practical machine learning settings, dataset sizes can be large, this can ultimately greatly degrade the quality of the odometer. Secondly, the tightness of the odometer greatly drops off outside of the interval $\left[ \frac{1}{|x|^2}, 1\right]$. In particular, in settings where the privacy parameters of algorithms being composed exceed $1$, the bound becomes many factors looser. Lastly, the form of the odometer is complicated. Ideally, a high-quality privacy odometer should have a straightforward dependence on $\sum_{m \leq n}\epsilon_m(x)^2$. 

To address the shortcomings of the privacy odometer in Fact~\ref{fact:rogers_odometers}, we use the various time-uniform concentration inequalities discussed in Section~\ref{sec:martingales:basics} to construct tighter privacy odometers. In particular, we will construct three types of odometers -- one from each of the concentration inequalities presented in Section~\ref{sec:martingales:basics}. These odometers, generally, all have advantages over the one presented above. First, the odometers all have fairly simple dependence on $\sum_{m \leq n}\epsilon_m(x)^2$, unlike the odometer presented in Fact~\ref{fact:rogers_odometers}. Second, the odometers have no dependence on the size of the underlying dataset, a desirable trait in the age of big data. Lastly, the odometers all have free parameters which can be fine-tuned/optimized for potential target levels of privacy.

\subsection{New Privacy Odometers}
\label{sec:odometers:new}

In the remainder of this section, we will always consider a sequence of algorithms $(A_n)_{n \in \N}$ all defined on some common probability space $(\Omega, \calF, \P)$. We will always have a collection $\{(\calF_n(x))_{n \in \N}\}_{x \in \calX}$ of filtrations of the underlying probability space and a collection of sequences of privacy parameters $\{(\epsilon_n(x), \delta_n(x))_{n \in \N}\}_{x \in \calX}$. We will always operate under the assumption that, for all $n \in \N$, algorithm $A_n$ is $(\epsilon_n, \delta_n)$-pDP conditioned on $\calF_{n - 1}$, as outlined in Definition~\ref{def:cpdp}. Lastly, for arbitrary $x \in \calX$, it will be useful to refer to the stopping time $N_{\delta}(x)$ given by
$$
N_{\delta}(x) = \inf\left\{ n \in \N : \delta < \sum_{m \leq n + 1}\delta_m(x)\right\}.
$$
This stopping time serves to indicate when the total sum of accumulated approximation parameters exceeds a predetermined threshold, allowing us to correspondingly trivialize the upper bound on privacy loss from that point forward (that is, make the upper bound $\infty$).

In some sense, constructing a privacy odometer is a problem we have already solved by investigating privacy filters. In particular, in our our proof of Theorem~\ref{thm:new_filter}, we already essentially constructed one form of odometer. We present said odometer in the following theorem.

\begin{theorem}[\textbf{Privacy Odometers from Filters}]
\label{thm:filter_odom}
Let $(A_n)_{n \in \N}$ be a sequence of algorithms such that $A_n$ is $(\epsilon_n, \delta_n)$-pDP conditioned on $\calF_{n - 1}$. Fix $\delta = \delta' + \delta'' > 0$, and let $\epsilon > 0$ be arbitrary. Let $N_{\delta''}(x)$ be the same $(\calF_n(x))_{n \in \N}$ be the stopping time outlined above. Let $y^\ast$ be the parameter used in optimizing the bound in Theorem~\ref{thm:new_filter}, i.e.
$$
y^\ast := \left(-\sqrt{2\log\left(\frac{1}{\delta'}\right)} + \sqrt{2\log\left(\frac{1}{\delta'}\right) + \epsilon}\right)^2,
$$
Then, we have that the collection of sequences $\{(U_n^F(x))_{n \in \N}\}_{x\in\calX}$ given by
$$
U_n^F(x) = \left[\frac{\sqrt{2y^\ast\log\left(\frac{1}{\delta'}\right)}}{2} + \frac{\sqrt{2y^\ast\log\left(\frac{1}{\delta'}\right)}}{2y^\ast}\sum_{m \leq n}\epsilon_m(x)^2 + \frac{1}{2}\sum_{m \leq n}\epsilon_m(x)^2\right]\one_{n \leq N_{\delta''}(x)} + \infty\one_{n > N_{\delta''}(x)}
$$
is a $\delta$-privacy odometer.

\end{theorem}

Observe that the above odometer is tightest when $\sum_{m \leq n}\epsilon_m(x)^2 \approx y^\ast$, and that the tightness drops off precipitously from there. As we will later graphically see, the estimates on privacy loss provided by $(U_n^F(x))_{n \in \N}$ are actually very loose for very small/large values of $\sum_{m \leq n}\epsilon_m(x)^2$. Nonetheless, if we know approximately a target overall level of privacy, these filter-based odometers will prove to be the tightest.

The remaining two odometers we will discuss sacrifice tightness at any fixed point in time to obtain an overall tighter bound on privacy loss.

To get a sense of how filter odometers look when optimized for various global values of $\epsilon > 0$, see Figure~\ref{fig:filter_odometers} below.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.5]{figures/filter_odom.png}
    \caption{Comparison of privacy odometers derived from privacy filters. We consider several values of $\epsilon$ and fix $\delta = \delta' = 10^{-6}$. We assume all algorithms being composed are purely differentially private for simplicity. The $x$-axis shows various potential values of $\sum_{m \leq n}\epsilon_m^2$, and the $y$-axis shows the corresponding bound on privacy loss. Note that no odometer strictly dominates another, demonstrating a tradeoff. }
    \label{fig:filter_odometers}
\end{figure}

We now develop a type of odometer which we call a \textit{stitched odometer}. The name derives from the method of stitched boundaries presented in~\cite{howard2021unif} to construct the time-uniform concentration inequality presented in Fact~\ref{fact:stitch}. Using this fact, we get the following general class of privacy odometer.

\begin{theorem}
\label{thm:stitch_odom} 
Suppose $(A_n)_{n \in \N}$ is a sequence of algorithms such that $A_n$ is $(\epsilon_n, \delta_n)$-pDP conditioned on $\calF_{n - 1}$. For any fixed $v_0 > 0$ and $\delta := \delta' + \delta'' > 0$, define the events $G_n(x)$ by
$$
G_n(x) := \left\{ \sum_{m \leq n}\epsilon_m(x)^2 \geq v_0,  n \leq N_{\delta''}(x)\right\}.
$$
Then, the collection $\{(U^S_n(x))_{n \in \N}\}_{x \in \calX}$ given by
$$
U^S_n(x) := \left[1.7\sqrt{\left(\sum_{m \leq n}\epsilon_m(x)^2\right)\left(\log\log\left(\frac{2\sum_{m\leq n}\epsilon_m(x)^2}{v_0}\right) + 0.72\log\left(\frac{5.2}{\delta'}\right)\right)} + \frac{1}{2}\sum_{m \leq n}\epsilon_m(x)^2\right]\one_{G_n(x)} + \infty \one_{G_n(x)^c}
$$
is a $\delta$-privacy odometer.
\end{theorem}



While the above odometer is a bit messy, it is significantly more readable than the odometer presented in Fact~\ref{fact:rogers_odometers}. The only catch is that the odometer requires that $\sum_{m \leq n}\epsilon_m(x)^2$ exceed some pre-selected ''variance" $v_0$ before the bound becomes nontrivial (i.e. finite). Larger values of $v_0$ will result in tighter odometers, albeit at the price of potentially losing validity of upper bounds when only a few algorithms are being composed. However, since $\epsilon_1(x)$ is always $\calF_{0}(x)$-measurable, and $\calF_0(x)$ is the trivial $\sigma$-algebra, we can always preselect $v_0 \geq \epsilon_1(x)^2$.

An important thing to note about the odometer presented in Theorem~\ref{thm:stitch_odom} is its rate. Namely, the rate is asymptotically optimal in the sense that it matches the law of the iterated logarithm up to constants and lower order terms. That is, $U_n^S(x) = O\left(\sqrt{\sum_{m \leq n}\epsilon_m(x)^2\log\log\left(\sum_{m \leq n}\epsilon_m^2\right)}\right)$. Thus, if we are composing \textit{many} algorithms -- all with large privacy parameters -- we in general expect this odometer to be the tightest. However, as we will discuss below and see in Figure~\ref{fig:odom_compare}, this does not mean that $(U_n^S(x))$ is the best privacy odometer for practical purposes. Since we often want to keep total level of privacy loss small, asymptotic performance is not, in general, a good metric for the quality of a privacy loss bound.

The fourth and final type of odometer we look at is what we call a mixture odometer. We give our odometer this name because it leverages Fact~\ref{fact:mixture}, a time-uniform concentration inequality derived from the so-called \textit{the method of mixtures}. For an exposition on the method of mixtures, we refer the reader to works such as \cite{balsubramani2014sharp,howard2021unif,kaufmann2018mixture,delapena2007maximization}.

We now apply Fact~\ref{fact:mixture} to construct our mixture privacy odometer in the following theorem.

\begin{theorem}[\textbf{Mixture Boundary Odometers}]
\label{thm:mixture}
Suppose $(A_n)_{n \in \N}$ is a sequence of algorithms such that $A_n$ is $(\epsilon_n, \delta_n)$-pDP given $\calF_{n - 1}$. Fix $\delta = \delta' + \delta'' \geq 0$ and an arbitrary $\rho > 0$. For any $x \in \calX$, define the bound $(B_n(x))_{n \in \N}$ by
$$
B_n(x) := \sqrt{2\log\left(\frac{1}{2\delta'}\sqrt{\frac{\sum_{m \leq n}\epsilon_m(x)^2 + \rho}{\rho}} + 1\right)\left(\rho + \sum_{m \leq n}\epsilon_m(x)^2\right)} + \frac{1}{2}\sum_{m \leq n}\epsilon_m(x)^2.
$$
Then, the collection of sequences $\{(U^B_n(x))_{n \in \N}\}_{x \in \calX}$ given by
$$
U^B_n(x) := B_n(x)\one_{n \leq N_{\delta''}(x)} + \infty \one_{n > N_{\delta''}(x)}
$$
is a $\delta$-privacy odometer.

\end{theorem}

We briefly compare the odometer in Theorem~\ref{thm:mixture} to the corresponding odometer in Theorem~\ref{thm:stitch_odom}. Then, we will compare the quality of all privacy odometers jointly. Note that the mixture odometer has worse asymptotic dependence on $\sum_{m \leq n}\epsilon_m(x)^2$ than the stitched odometer. Nonetheless, we will come to see that the mixture odometer is often empirically much tighter, especially for small values of $\sum_{m \leq n}\epsilon_m(x)^2$. Moreover, unlike the stitched odometer, there is no tradeoff between the variance at which the bound becomes valid and the tightness of the odometer. 


\subsection{Comparison of Privacy Odometers}
\label{sec:odometers:comparison}

With our four classes of privacy odometers constructed, we now make several qualitative comparisons. At first glance, the privacy odometer in Theorem~\ref{thm:stitch_odom} seems to be the most preferable as it has the best asymptotic rate. In particular, the former stitched odometer has an asymptotic rate of $$O\left(\sqrt{\log\log\left(\sum_{m \leq n}\epsilon_m^2\right)\sum_{m \leq n}\epsilon_m^2}\right).$$ On the other hand, both the original privacy odometer and the mixture odometer have a rate of $$O\left(\sqrt{\log\left(\sum_{m \leq n}\epsilon_m^2\right)\sum_{m \leq n}\epsilon_m^2}\right),$$ and the original odometer also has a dependence on dataset size $|x|$. In addition, the odometer obtained from privacy filters grows at a linear rate of $O\left(\sum_{m \leq n}\epsilon_m^2\right)$. Nonetheless, this does not mean the stitched odometer is the best overall choice. In particular, there are many ranges of $\sum_{m\leq n}\epsilon_m^2$ for which any given odometer outperforms the others. This demonstrates that selecting a privacy odometer for a given problem is actually a very subtle manner, depending on the goal of the underlying experiment.

Now, we empirically compare the four odometers presented above. To compactly do so, we make several observations about the aforementioned odometers. First, observe that, to compare the odometers, it suffices to just consider \textit{purely} differentially private algorithms, as the odometers all depend on the approximation sequence $(\delta_n)_{n \in \N}$ trivially in the same way. Second, note that each presented odometer can be viewed as a function of the sum of squares of privacy parameters, $\sum_{m \leq n}\epsilon_m^2$. As such, instead of creating plots for various choices of sequences $(\epsilon_n)_{n \in \N}$, it really suffices just to plot corresponding privacy loss bound values for a continuum of values of $y := \sum_{m \leq n}\epsilon_m^2$. Lastly, several of the odometers (e.g. mixture and filter odometers) can, in a sense, be optimized for various points in time. As such, to do a proper comparison, in a given graphic, we always optimize said odometers for the same point in time, as we feel this gives the best understanding of how the odometers globally compare.

\begin{figure}
    \centering
    \includegraphics[width=.32\textwidth]{figures/linear_100.0.png}
    \includegraphics[width=.32\textwidth]{figures/linear_10000.0.png}
    \includegraphics[width=.32\textwidth]{figures/linear_1000000.0.png}
    \caption{Comparing all four odometers as functions of $\sum_{m \leq n}\epsilon_m^2$. The filter odometer is set at $\epsilon = 8$, the mixture odometer is set at $\rho = 0.01$, and the stitched odometer is taken with variance term $v = 0.01$. Other values are possible, but we present these for illustrative purposes. We vary the number of data points $n$ included in the dataset for the original odometers.}
    \label{fig:odom_compare}
\end{figure}

Looking at Figure~\ref{fig:odom_compare}, we see that there is no clearly dominant odometer in terms of tightness. All odometers, barring the original odometer presented in Rogers et al.~\cite{rogers2016odometer}, is dominant for some window of values of $\sum_{m \leq n}\epsilon_m(x)^2$. Even though the stitched odometer achieves the best asymptotic rate, the mixture odometer is tighter for small values of $\sum_{m \leq n}\epsilon_m(x)^2$. Likewise, if one has very good knowledge of a rough target of overall privacy loss, the filter odometer may prove to be the tightest option.


==> Old_Tex/PrivacyOLD.tex <==
\section{Mathematical Background}
\label{sec:background}

In this section, we cover the basics of differential privacy from a measure-theoretic perspective. Although the formalism of measure theory requires more background knowledge on the part of the reader, it allows for a rigorous study of the composition of differentially private algorithms. To combat the increased level of formalism, we often provide a verbal interpretation of definitions after presenting them.

Before proceeding with a measure-theoretic interpretation of differential privacy, we present some notation and some basics of measure theory.

\subsection{Notation and Measure-Theoretic Preliminaries}
\label{sec:background:notation}

\paragraph{Neighboring Datasets:} 
The simple idea behind differential privacy is that a randomized algorithm is private if minor perturbations to inputs only result in minor perturbations of output distributions. In general, this notion of similarity is defined as a \textit{neighboring relation} $\sim$ between elements on the space of algorithm input $\calX$s. In particular, if two inputs (also referred to as datasets or databases) $x, x' \in \calX$ satisfy the neighboring relation $x \sim x'$, the we say $x$ and $x'$ are \textit{neighbors}. 

There are several canonical examples of neighboring relations on the space of inputs $\calX$. As one example is where $\calX = \mathbb{X}^n$ for some data domain $\mathbb{X}$. The data domain can be viewed as the set of all possible individual entries for a dataset, and the space $\mathbb{X}^n$ correspondingly contains all possible $n$ element datasets. In this setting, databases $x, x' \in \calX$ may be considered neighbors if $x$ and $x'$ differ in exactly one entry. Another slightly more general setting is when $\calX = \mathbb{X}^*$, i.e. $\calX$ contains all possible datasets of finite size. In this situation, the earlier notion of neighboring still makes sense. However, in addition, we may say input datasets $x$ and $x'$ are neighbors if $x$ can be obtained from $x'$ by either adding or deleting an element. This is a very natural notion of neighboring, as under such a relation an algorithm would be differentially private if it were difficult to determine whether or not any given individual was present in the datset. Overall, in the context of this work, the exact implementation of the neighboring relation $\sim$ is unimportant. As such, we choose to leave the notion as general as possible.

\paragraph{Algorithms and Random Variables:} We will consider algorithms as randomized mappings $A : \calX \rightarrow \calY$ taking inputs from $\calX$ to some output space $\calY$. To be fully formal, we consider the output space $\calY$ as a \textit{measurable space} $(\calY, \calG)$, where $\calG$ is some $\sigma$-algebra denoting possible events. Recall that a $\sigma$-algebra $\calS$ for a set $S$ is simply a subset of $2^S$ containing $S$ and $\emptyset$ that is closed under countable union, intersection, and complements. To formalize the randomness used in an algorithm $A$, for any $x \in \calX$, we can view $A(x)$ as a random variable $A(x) : \Omega \rightarrow \calY$ taking values from some shared probability space $(\Omega, \calF, \P)$ (where $\calF$ is a $\sigma$-algebra and $\P$ a probability measure) to outputs in the measurable space $(\calY, \calG)$. Heuristically, inputs $\omega \in \Omega$ can be viewed as the ''seed" for the randomness in the algorithm $A$. As is standard, in most settings we drop the explicit notational dependence on inputs $\omega \in \Omega$, writing $A(x)$ in place of $A(x)(\omega)$. Even in settings where we have a sequence of algorithms $(A_n)_{n \in \N}$, we assume that all random variables are defined on a shared probability space and take outputs in the same space, i.e. $A_n(x)$ is a $\calY$-valued random variable on $(\Omega, \calF, \P)$ for all $n \in \N$, $x \in \calX$. Even if algorithms have different types of outputs (maybe some algorithms have categorical outputs while others output real-valued vectors), $\calY$ can still be made appropriately large to contain all possible outcomes. 

Since we are dealing with the composition of algorithms, we write $A_{1:n}(x)$ as shorthand for the random vector of the first $n$ algorithm outputs, i.e. $A_{1:n}(x) = (A_1(x), \dots, A_n(x))$. The random vector $A_{1:n}(x)$ takes output values in the product measurable space $(\calY^n, \calG^{\otimes n})$ where $\calG^{\otimes n}$ denotes the $n$-fold product $\sigma$-algebra of $\calG$ with itself. Likewise, since the number of algorithm outputs one views in fully-adaptive composition may be random, if $N$ is a random time (i.e. a $\N$-valued random variable), we will often consider the random vector $A_{1:N}(x) = (A_1(x), \dots, A_N(x))$. To make our lives easy, we can view $A_{1:N}(x)$ as a random vector in the infinite product output space $(\calY^\infty, \calG^{\otimes \infty})$. We do this by simply inserting a special terminating element $\square$ into $\calY$ and repeating it ad infinitum after the last element of the random vector, i.e. $A_{1:N}(x) = (A_1(x), \dots, A_N(x), \square, \square, \dots)$. The reader should not concern himself with the detail here -- we just include this information to be fully formal and so it is explicit which sets of outcomes are considered measurable.

Lastly, we always make the assumption that the measurable space of algorithm outputs $(\calY, \calG)$ is \textit{nice} \cite{durrett2019probability}, i.e. that either $\calY$ is discrete and $\calG = 2^\calY$ or that there is a bi-measurable bijection between $\calY$ and $\R$ where we view $\R$ as being equipped with the Borel $\sigma$-algebra $\calB(\R)$ (that is, the $\sigma$-algebra generated by the open sets of $\R$ under the standard topology). In particular, if $\calY = \R^d$ and $\calG = \calB(\R^d)$ for some integer $d \geq 1$, then $(\calY, \calG)$ is nice. We consider this notion of regularity on the space of outputs because it guarantees the existence of regular conditional probabilities. Given a sub $\sigma$-algebra $\calF' \subset \calF$, a \textit{regular conditional probability} is a probability kernel $\mu_{\calF'} : \Omega \times \calG \rightarrow [0, 1]$ such that for any fixed $\omega \in \Omega$, $\mu_{\calF'}(\omega, \cdot)$ is a probability measurable on the space $(\calY, \calG)$. Regular conditional probabilities are essential for defining conditional versions of privacy loss, as one can use regular conditional probabilities to construct conditional densities for the algorithms being composed.

\paragraph{Filtrations and Stopping Times:} Given that we will be considering sequences of random outputs, it is sometimes necessary to discuss the measure-theoretic notion of a \textit{filtration}. Given some probability space $(\Omega, \calF, \P)$, a filtration $(\calF_n)_{n \in \N}$ for $\calF$ is a sequence of $\sigma$-algebras satisfying: (i) $\calF_n \subset \calF_{n + 1}$ for all $n \in \N$, and (ii) $\calF_n \subset \calF$ for all $n \in \N$. Given an arbitrary $\calY$-valued discrete-time stochastic process $(X_n)_{n \in \N}$, it is often useful to get consider the filtration $(\calF_n)_{n \in \N}$ given by $\calF_n := \sigma(X_m : m\leq n)$. Such a filtration is called the \textit{natural filtration} of $\calF$ associated with $(X_n)_{n \in \N}$, as $\calF_n$ entails all possible events determined by the first $n$ iterates of the stochastic process $(X_n)_{n \in \N}$. Intuitively, a filtration formalizes the notion of accumulating information over time. In particular, in the context of the natural filtration of a stochastic process, the $n$th $\sigma$-algebra in the filtration $\calF_n$ essentially represents the entirety of information contained in the first $n$ random variables. In other words, if one is given $\calF_n$, they would know all possible events/outcomes that could have occurred up to and including timestep $n$.

Lastly, we briefly mention the notion of a \textit{stopping time}, as this measure-theoretic object is necessary to define privacy filters. Given a filtration $(\calF_n)_{n \in \N}$, a random time $N$ is said to be a stopping time with respect to $(\calF_n)_{n \in \N}$ if, for any $n$, the event $\{N \leq n\} \in \calF_n$. In words, a random time $N$ is a stopping time if given the information in $\calF_n$ we can determine whether or not we should have stopped by time $n$. Stopping times are essential to the study of fully-adaptive composition, as a practitioner of privacy will need to use the adaptively selected privacy parameters to determine whether or not to stop interacting with the underlying sensitive database. This interactive stopping, as we will see, is necessary to maintain overall global desired levels of privacy. 


\subsection{Conditional Differential Privacy}
\label{sec:background:dp}

As alluded to in the Introduction, a randomized algorithm is differentially private if similar inputs induce similar distributions over outputs. This seemingly high-level definition is formalized in the following pioneering definition \cite{dwork2006priv}.

\begin{definition}
\label{def:dp}
A randomized algorithm $A$ mapping inputs from a space $\calX$ to a measurable space $(\calY, \calG)$ is said to be $(\epsilon, \delta)$-differentially private if, for any neighboring inputs $x \sim x' \in \calX$ and any measurable set $G \in \calG$, we have
$$
\P(A(x) \in G) \leq e^\epsilon\P(A(x') \in G) + \delta.
$$
\end{definition}

From Definition~\ref{def:dp}, researchers have been able to construct an arsenal of private data analysis techniques. Many of these techniques, especially those related to optimization procedures \cite{wang2019subsampled} \cite{song2013stochastic} rely on the fact that differentially private algorithms compose gracefully. Given a algorithms $A_1, \dots, A_k$, the \textit{composed} algorithm $A_{1:k}$ is the mechanism which, on input $x$, release $A_1(x), \dots, A_k(x)$. In other words,
$$
A_{1:k}(x) := (A_1(x), \dots, A_k(x)).
$$
More on the idea of algorithm composition and the corresponding notation can be found in Section~\ref{sec:background:notation}. The following folklore theorem, known as \textit{Advanced Composition}, gives our point of comparison for fully-adaptive composition \cite{dwork2010boosting} \cite{kairouz2015composition} \cite{murtagh2016complexity}.

\begin{fact}[\textbf{Advanced Composition}]
\label{fact:adv_comp}
Suppose $A_1, \dots, A_k$ are algorithms mapping inputs from $\calX$ to outputs in the measurable space $(\calY, \calG)$. Suppose, for all $i \in [k]$, algorithm $A_i$ is $(\epsilon_i, \delta_i)$-differentially private, and let $\delta' > 0$ be arbitrary. Then, the composed algorithm $A_{1:k}$ is $(\epsilon, \delta)$-differentially private, where
$$
\epsilon = \sqrt{2\log\left(\frac{1}{\delta'}\right)\sum_{m \leq k}\epsilon_m^2} + \frac{1}{2}\sum_{m \leq k}\epsilon_m\left(\frac{e^{\epsilon_m} - 1}{e^{\epsilon_m} + 1}\right) \qquad \delta = \delta' + \sum_{m \leq k} \delta_m.
$$
\end{fact}

Note that neither Definition~\ref{def:dp} nor Fact~\ref{fact:adv_comp} allow for the privacy parameters $\epsilon_i$ and $\delta_i$ to be random quantities depending on the outputs of previous algorithms. To capture this more general case of adaptive privacy parameter selection, the definition of privacy fundamentally needs to be extended to handle the accumulation of information over time.

Our goal going forward is to develop (and interpret) an extension to the definition of differential privacy to allow the privacy parameters to depend on potentially random auxiliary information. For full generality, this information can be anything. For instance, it can be the outcome of independent coin flips, a draw from a Gaussian distribution, or even the random outcomes of previous algorithms. To allow the privacy parameters to be functions of random variables, we replace the probabilities in Definition~\ref{def:dp} with conditional probabilities where we condition on the sigma algebra generated by the information we want to be available to the data analyst. There are several subtleties to doing this, which we ellaborate upon below.

\begin{definition}[\textbf{Conditional Differential Privacy}]
\label{def:cdp}
Suppose $A$ is an algorithm having inputs in a space $\calX$ and outputs in a measurable space $(\calY, \calG)$. In other words, for any $x \in \calX$, assume $A(x)$ is a random variable defined on a probability space $(\Omega, \calF, \P)$.  Suppose $\{(\epsilon(x), \delta(x))\}_{x\in\calX}$ is a set of tuples of privacy parameters, and $\{\calH(x)\}_{x \in \calX}$ is a set of sub sigma-algebras of $\calF$. We say the algorithm $A$ is $\{(\epsilon(x), \delta(x))\}$-differentially private conditioned on $\{\mathcal{H}(x)\}_{x \in \calX}$ (or, for shorthand, the algorithm $A$ is $(\epsilon, \delta)$-differentially private conditioned on $\mathcal{H}$) if
\begin{enumerate}
    \item for any $x \in \calX$, $\epsilon(x)$ and $\delta(x)$ are $\calH(x)$-measurable random variables, and
    \item for any neighboring datasets $x \sim x' \in \calX$ and for all measurable sets $G \in \calG$, we have
    $$
    \P\left(A(x) \in G\mid\calH(x)\right) \leq e^{\epsilon(x)}\P\left(A(x') \in G \mid \calH(x')\right) + \delta(x).
    $$
\end{enumerate}

\end{definition}

Definition~\ref{def:cdp} may seem abstract, but the formalization is important. We can make sense of the definition and justify the level of formality through the example of adaptive composition. In adaptive composition, we typically view an analyst as having a sequence of adaptively chosen algorithms $(A_n)_{n \in \N}$. If this sequence of algorithms takes as inputs in some set $\calX$, we can equivalently view the analyst as having access to a sequence of random variables, $(A_n(x))_{n \in \N}$. For each fixed $x \in \calX$, the sequence $(A_n(x))_{n \in \N}$ may admit some complicated joint distribution between elements of the sequence, capturing the fact that the choice of the algorithms may be adaptive. 

In terms of selecting privacy parameters, we can view the analyst as having two sequences of functions, $(\mathcal{E}_n)$ and $(\Delta_n)$, where $\mathcal{E}_n, \Delta_n :\calY^{n - 1} \rightarrow \R_{\geq 0}$ are $\calG^{\otimes n - 1}$-measurable (assuming $\R_{\geq 0}$ is made into a measurable space by endowing it with the Borel-sigma algebra). In plain English, the analyst uses the outcome of the first $n-1$ algorithms to decide the level of privacy for the $n$th algorithm. 

For each $x \in \calX$, we will consider the natural filtration $(\calF_n(x))_{n \in \N}$, where $\calF_n(x) := \sigma(A_k(x) : k \leq n)$ is the sigma-algebra generated by the outputs of the first $n$ algorithms acting on input $x$. A filtration is just a sequence of sigma algebras $(\calF_n)_{n \in \N}$ such that, for all $n \in N$, $\calF_n \subset \calF$ and $\calF_n \subset \calF_{n + 1}$. Consequently, the analyst will pick the privacy parameters $\epsilon_n(x), \delta_n(x) :\Omega \rightarrow \R_{\geq 0}$ according to the composed rules
$$
\epsilon_n(x) := (\mathcal{E}_n \circ A_{1:n-1}(x)) \qquad \text{and} \qquad \delta_n(x) := (\Delta_n \circ A_{1:n-1}(x)).
$$

Observe that, since compositions of measurable maps are measurable, $\epsilon_n(x)$ and $\delta_n(x)$ are $\calF_{n - 1}(x)$-measurable, as necessitated by the definition of conditional privacy. Note that the $x$ in the notation is just for the purpose of indexing. The analyst need not know (and indeed, does not know) which input $x$ is generating the data, but it is the case (and is natural) that the distribution of observed privacy parameters does in fact depend on the underlying $x$.

Consequently, for each $n \in \N$, it makes sense to assume that the analyst desiring privacy in each round would ensure the $n$th algorithm $A_n$ is $\{(\epsilon_n(x), \delta_n(x))\}_{x \in \calX}$-differentially private conditioned on $\{\calF_{n - 1}(x)\}_{x \in \calX}$, or, in terms of our simplified notation, that $A_n$ is $(\epsilon_n, \delta_n)$-differentially private conditioned on $\calF_{n - 1}$.

Lastly, before moving on, we discuss a key property of differential privacy: closure under post-processing. In particular, if $A : \calX \rightarrow \calY$ is an $(\epsilon, \delta)$-differentially private algorithm and $f : \calY \rightarrow \calZ$ is a random function which is \textit{independent} of $A(x)$, for all $x \in \calX$, then the the algorithm $B : \calX \rightarrow \calZ$ given by $B(x) = f(A(x))$ is in fact  $(\epsilon, \delta)$-differentially private as well \cite{dwork2014algorithmic}. We will need to the following straightforward extension of this result.

\begin{lemma}
\label{lem:post_process}
Let $A$ be an algorithm taking inputs in a space $\calX$ to outputs in a measurable space $(\calY, \calG)$. Let $\{(\epsilon(x), \delta(x))\}_{x \in \calX}$ be a family of privacy parameters, $\{\calH(x)\}_{x \in \calX}$ a family of $\sigma$-algebras, and $\{f_x\}_{x \in \calX}$ a collection of functions from $\calY$ to $\calZ$, for some measurable space $(\calZ, \calS)$. Suppose $A$ is $(\epsilon, \delta)$-differentially private given $\calH$, and assume that $f_x$ is independent of $A(x')$ given $\calH(x)$, for all $x, x' \in \calX$. Then, the algorithm $B$ given by $B(x) = f_x(A(x))$ is $(\epsilon, \delta)$-differentially private given $\calH$.
\end{lemma}

The proof of Lemma~\ref{lem:post_process} is identical to the proof of typical closure under post-processing where regular probabilities are replaced by the corresponding conditional ones. Consequently, we omit the proof.

\subsection{Conditional and Composed Privacy Loss}
\label{sec:background:ploss}
It is difficult to directly prove composition results for differential privacy by directly working the above definitions. Instead, the \textit{privacy loss} random variable becomes central to proving privacy composition results \cite{dwork2014algorithmic} \cite{kairouz2015composition} \cite{rogers2016odometer}. On an intuitive level, privacy loss is a measure of how much information is revealed about which underlying dataset is being used at any step in computation. At a slightly more formal level, before computation, an analyst selects two neighboring datasets, $x, x' \in \calX$. The privacy loss is then a log-likelihood ratio, giving the bias a data analyst would have toward whether the witnessed outputs were produced by an input $x$ or a similar input $x'$. When privacy loss is very negative, an analyst would believe $x'$ was the underlying dataset. Likewise, if privacy loss were high, the analyst would be biased toward to the input $x$. We define privacy loss as follows.
\begin{definition}[\textbf{Privacy Loss}]
\label{def:ploss}
Suppose $A$ is a randomized algorithm mapping taking inputs in a space $\calX$ and outputs in a measurable space $(\calY, \calG)$. Let $x$ be a fixed input, and $x' \sim x \in \calX$ a fixed alternative. Let $\nu$ be a $\sigma$-finite reference measure on $(\calY, \calG)$ such that the laws of $A(x)$ and $A(x')$ are absolutely continuous with respect to $\nu$. Correspondingly, let $p^x$ and $p^{x'}$ be the densities for the laws of $A(x)$ and $A(x')$ with respect to $\nu$. Then, \textit{privacy loss between $A$ run on $x$ and $A$ run on $x'$} is the random variable $\calL(x, x')$ given by
$$
\calL(x, x') := \log\left(\frac{p^x(A(x))}{p^{x'}(A(x))}\right).
$$

\end{definition}

Definition~\ref{def:ploss} essentially just formalizes the intuitive definition of privacy loss presented in the previous paragraph. The next definition, that of \textit{conditional privacy loss}, takes the same intuition and maps it to the setting where an analyst may have additional information which may guide their decisions. 

We need to extend our assumptions to formalize conditional privacy loss. As in the definition of privacy loss, we fix a reference measure $\nu$ on $(\calY, \calG)$ such that, for any $x \sim x' \in \calX$, the regular conditional probabilities of $A(x)$ and $A(x')$ respectively admit conditional densities $p_x$ and $p_{x'}$ with respect to $\nu$ conditioned on $\calH(x)$, where $\calH(x)$ is a sigma algebra containing additional information.
%Once again, for a background on measure-theoretic concepts such as regular conditional probabilities and conditional densities, please refer to Appendix~\ref{}.

\begin{definition}[\textbf{Conditional Privacy Loss}]
\label{def:cploss}
Suppose $A$ is an algorithm mapping inputs from a space $\calX$ to the measurable space $(\calY, \calG)$.  Suppose there is a collection of $\sigma$-algebras $\{\calH(x)\}_{x \in \calX}$ and suppose $x \sim x' \in \calX$ are neighboring datasets. Let $\mu^x_{\calH(x)}, \mu^{x'}_{\calH(x)}: \Omega \times \calG \rightarrow [0, 1]$ be the regular conditional probabilities for $A(x)$ and $A(x')$ respectively given $\calH(x)$. Let $\nu : \Omega \times \calG \rightarrow [0, 1]$ be a $\sigma$-finite regular conditional probability measure on $(\calY, \calG)$ such that, for all $\omega \in \Omega$, $\mu^x_{\calH(x)}(\omega, \cdot), \mu^{x'}_{\calH(x)}(\omega, \cdot) << \nu(\omega, \cdot)$. Let $p^x, p^{x'} : \Omega \times \calY \rightarrow \R_{\geq 0}$ be corresponding (random) conditional densities for $\mu^{x}_{\calH(x)}$ and $\mu^{x'}_{\calH(x)}$ with respect to $\nu$. Then, the \textit{conditional privacy loss of algorithm $A$ between inputs $x$ and $x'$ given $\calH(x)$} is defined as the random variable $L_{\calH}(x, x'): \Omega \rightarrow \R$ given by
$$
\calL_{\calH}(x, x')(\omega) := \log\left(\frac{p^x_{\calH(x)}(\omega, A(x))}{p^{x'}_{\calH(x)}(\omega, A(x))}\right),
$$
where the outcome $A(x) = A(x)(\omega)$ implicitly depends on $\omega \in \Omega$.

\end{definition}

We once again contextualize the above definition in the setting of sequential composition. Let $(A_n)_{n \in \N}$ be a sequence of adaptively chosen algorithms. Moreover, suppose we are considering the $n$th algorithm $A_n$ in the sequence. We have already observed $A_{1:n-1}(x)$ for some unknown input $x \in \calX$, and we are trying to determine whether dataset $x \in \calX$ produced the data, or another dataset $x' \in \calX$. To determine our bias as to whether $x$ or $x'$ produced the data, we want to consider the privacy loss between $A_n(x)$ and $A_n(x')$ conditioned on $\calH(x) := \calF_{n -1}(x) = \sigma(A_k(x) : k \leq n -1)$ (that is, conditioned on the output of the first $n - 1$ algorithms). We leave the definition to be broader than this specific setting for full generality. However, in this special case of composed interactions, we refer to the privacy loss in the $n$th round conditioned on $\calF_{n - 1}(x)$ as
$$
\calL_{n}(x, x') := \calL_{\calF_{n - 1}(x)}(x, x')
$$
to simplify notation.

One reason differential privacy researchers study privacy loss is that it is easy to characterize the privacy loss of a composed algorithm $A_{1:n}$ by studying the conditional privacy loss of each constituent algorithm $A_1, \cdots, A_n$. Namely, we have the following fact which follows directly from Bayes rule.

\begin{fact}[\textbf{Privacy Loss of Composed Algorithms}]
\label{fact:ploss_comp}
Suppose $(A_n)$ is an adaptively chosen sequence of algorithms. Let $x \sim x' \in \calX$ be neighboring datasets. Then, for any $n \in \N$, the privacy loss between $A_{1:n}(x)$ and $A_{1:n}(x')$, denoted $\calL_{1:n}(x, x')$, satisfies
\(
\calL_{1:n}(x, x') = \sum_{m \leq n}\calL_{m}(x, x'),
\)
where $\calL_m(x, x')$ is conditional privacy loss between $A_m(x)$ and $A_m(x')$ given $\{\calF_{m - 1}(x)\}_{x \in \calX}$, per Definition~\ref{def:cploss}.
Thus, if $N(x)$ is a $(\calF_{n}(x))_{n \in \N}$-stopping time, the privacy loss between $A_{1:N(x)}(x)$ and $A_{1:N(x')}(x')$ satisfies
$$
\calL_{1:N(x)}(x, x') = \sum_{m \leq N(x)}\calL_m(x, x').
$$
\end{fact}

Due to the simple decomposition of privacy loss in Fact~\ref{fact:ploss_comp}, studying the privacy of composed algorithms boils down to studying the concentration of privacy loss random variables. We discuss in detail studying the concentration of said random variables in Sections~\ref{sec:martingales:ploss} and \ref{sec:filter}. Definitions~\ref{def:ploss} and \ref{def:cploss} both suggest an alternative way to define the concept of differential privacy. We now discuss this in the following subsection.

\subsection{Probabilistic Differential Privacy}
\label{sec:background:pdp}

We now discuss another notion of privacy, which we refer to as \textit{probabilistic differential privacy}. We motivate this notion of privacy by considering an ``alternative'' definition of differential privacy which leverages privacy loss. Informally, an algorithm should be $(\epsilon, \delta)$-differentially private if, with probability $\geq 1 - \delta$, the privacy loss is bounded above by $\epsilon$. This would provide an additional, more intuitive meaning to Definition~\ref{def:dp}. Unfortunately, the above alternative definition is not, in general, equivalent to differential privacy. However, when considering problems such as privacy composition, this notion is much easier to work with, as it gives us a means of directly applying concentration inequalities. We formalize this alternative notion of privacy as follows.

\begin{definition}[\textbf{Probabilistic Differential Privacy}]
\label{def:pdp}
A randomized algorithm $A$ mapping values in some space $\calX$ to some measurable space $(\calY, \calG)$ is said to be $(\epsilon, \delta)$-\textit{probabilistically-differentially private}, or $(\epsilon, \delta)$-pDP for short, if, for all neighboring inputs $x \sim x' \in \calX$, the privacy loss $\calL(x, x')$ satisfies
$$
\P\left( \calL(x, x') > \epsilon \right) \leq \delta.
$$

\end{definition}

The concept of probabilistic differential privacy is introduced and discussed in detail in \cite{kasiviswanathan2014semantics}. While the authors refer to the notion as \textit{semantic differential privacy}, we opt for probabilistic differential privacy due to the more intuitive nature of the latter term. The authors in \cite{kasiviswanathan2014semantics} explicitly demonstrate that probabilistic differential privacy is a strictly stronger notion than differential privacy. In particular, if an algorithm is $(\epsilon, \delta)$-probabilistically differentially private, it is also $(\epsilon, \delta)$-differentially private. The converse, in general, unfortunately is not true. Instead, a potentially costly conversion is required. We outline this in the following Lemma which can be found in \cite{kasiviswanathan2014semantics}.

\begin{lemma}[\textbf{Conversions between DP and pDP}]
\label{lem:dp_to_pdp}
Let $A$ be a randomized algorithm taking inputs in $\calX$ to outputs in a measurable space $(\calY, \calG)$. If $A$ is $(\epsilon, \delta)$-probabilistically differentially private, the $A$ is also $(\epsilon, \delta)$-differentially private. Conversely, if $A$ is $(\epsilon, \delta)$-differentially private, then $A$ is $(2\epsilon, \frac{2\delta}{\epsilon e^\epsilon})$-probabilistically differentially private.
\end{lemma}

In this work, we will be proving most results on the level of probabilistic differential privacy, and hence will only ever need the cost-free forward conversion between the notions of privacy. Thus, we will avoid needing to the pay the potentially unbounded conversion cost in the converse direction of Lemma~\ref{lem:dp_to_pdp}. In Section~\ref{sec:fully_adaptive}, we do handle the case where the algorithms being composed are conditionally differentially private. However, instead of relying on Lemma~\ref{lem:dp_to_pdp} to reduce to probabilistic privacy, we leverage an extension of the fact that differentially private algorithms can be viewed as a randomized post-processing of the randomized response mechanism \cite{kairouz2015composition} \cite{murtagh2016complexity}.

As with the definition of differential privacy discussed in Section~\ref{sec:background:dp}, probabilistic differential privacy admits a natural conditional counterpart for a setting in which an analyst may be composing algorithms.

\begin{definition}[\textbf{Conditional Probabilistic Differential Privacy}]
\label{def:cpdp}
An algorithm $A$ taking inputs in a space $\calX$ to outputs in a measurable space $(\calY, \calG)$ is said to be $\{(\epsilon_n(x), \delta_n(x))\}_{x\in\calX}$-\textit{conditionally probabilistically differentially private} with respect to a collection of sigma algebras $\{\calH(x)\}_{x \in \calX}$, or conditionally $(\epsilon_n, \delta_n)$-pDP for short if 
\begin{enumerate}
    \item $\epsilon_n(x)$ and $\delta_n(x)$ are $\calH(x)$-measurable random variables for all $x \in \calX$, and
    \item for any neighboring inputs $x \sim x'$, we have
    $$
    \P\left(\calL_{\calH(x)}(x, x') > \epsilon_n(x) | \calH(x)\right) \leq \delta_n(x),
    $$
\end{enumerate}
where $\calL_{\calH(x)}(x, x')$ is the conditional privacy loss random variable defined in Definition~\ref{def:cploss}.
\end{definition}

Once again, in the composed setting with a sequence of algorithms $(A_n)_{n \in \N}$, we assume $A_n$ is conditionally $(\epsilon_n, \delta_n)$-pDP with respect to a collection sigma algebras $\{\calF_{n - 1}(x)\}_{x \in \calX}$ containing the natural sigma algebras generated by the first $n - 1$ algorithm outputs, i.e. $\calF_{n - 1}(x) = \sigma(A_k(x) :k \leq n - 1)$. Much of the intuition behind Definition~\ref{def:cpdp} follows from the intuitive interpretation of conditional differential privacy following Definition~\ref{def:cdp}, so we refer the reader there for further motivation (e.g., how to view the random variables $\epsilon_n(x)$ and $\delta_n(x)$, for instance).

We have now completed our presentation of differential privacy, privacy loss, and related notions. We mentioned above that it is beneficial to study privacy loss random variables because we can ultimately apply concentration of measure results to prove overall privacy levels. As such, in the next section, we lay our framework for doing exactly this. 


==> Old_Tex/TechnicalResults.tex <==
\section{Closure of Conditional Differential Privacy under Post-Processing}

In this section, we provide a conditional analogue for the folklore result that differential privacy is closed under ``arbitrary" randomized post-processing. We put quotations around the word arbitrary to really emphasize that there are, in fact, strict limitations on the random functions under the standard proof of closure presented in Dwork et al.~\cite{dwork2014algorithmic}. In general, the random post-processing function must be \textit{independent} of the random variable $A(x)$ for all $x \in \calX$. 

While this requirement of independence seems innocuous, it makes studying differential privacy in our sequential setting much more difficult. In particular, even though we may know that a composed interaction/algorithm $A_{1:N(\cdot)}(\cdot)$ is $(\epsilon, \delta)$-differentially private, the usual closure under post-processing result does not permit us to post-process $A_n(x)$ in a random manner that depends on the first $n - 1$ post-processed outcomes. \rrcomment{This subtlety needs to be hammered down a bit more here.  In particular, what is wrong with considering $\Pr[f(A_2(x,A_1(x))) = y] = \sum_{a} \Pr[f(A_2(x,a)) = y | A_1(x) = a] * \Pr[A_1(x) = a]$, and now $f$ should be independent of $A_2(x,a)$ for any $a$ and $x$.  Is there something that goes wrong when we are considering post-processed values of $A_1(x)$ here? Or is it about how when $\delta>0$ we need to consider outcome sets?} In this appendix, we demonstrate that this sort of post-processing is, in fact, allowed.

Before we state the formal post-processing guarantee, we present another way to view randomized post-processing through probability transition kernels. Typically, one would consider a random function as a randomized mapping $f : \Omega \times \calY \rightarrow \calZ$ where $(\Omega, \calF, \P)$ is a shared, underlying probability space, $(\calY, \calG)$ is a space of outputs for an algorithm $A$, and $(\calZ, \calH)$ is a space of outputs for the random mapping $f$. This approach is somewhat clunky, and generalizes poorly to the setting where one may have a sequence of functions $(f_n)_{n \in \N}$ with some complicated dependence structure. We opt for the simpler approach of viewing randomized post-processing through transition kernels.

In its simplest form, we can view a probability transition kernel as a mapping $k : \calH \times \calY \rightarrow [0, 1]$ such that 
\begin{enumerate}
    \item for any $y \in \calY$, $k(\cdot, y)$ is a probability measure on $(\calZ, \calH)$, and
    \item for any $H \in \calH$, $k(H, \cdot) : \calY \rightarrow [0, 1]$ is a measurable function when $[0, 1]$ is equipped with the Borel sets.
\end{enumerate}

Note that this notion of a probability transition kernel is essentially equivalent to the earlier presented notion of a regular conditional probability \textit{except} that a transition kernel has no dependence on the underlying probability space $(\Omega, \calF, \P)$. This is useful for our purposes, as it will allow us to avoid notions of independence on the underlying probability space and instead work directly with the laws of the algorithms being composed.

To illustrate how one can use such probability kernels to represent post-processing, we re-state and re-prove the standard closure under arbitrary post-processing result. The only caveat we will face going forward is that we will need to assume that the algorithm being post-processed satisfies \textit{probabilistic} differential privacy, as outlined in Section~\ref{sec:background:pdp}. While this is a strictly stronger assumption than that of differential privacy, it suffices for our study in this paper. In particular, the only time we will need to apply our post-processing result is to post-process the outputs of conditional randomized-response, which satisfy conditional probabilistic differential privacy.

\begin{lemma}
\label{lem:clos_pp}
Let $A$ be a randomized algorithm taking inputs from $\calX$ to outputs in the measurable space $(\calY, \calG)$. Suppose algorithm $A$ is $(\epsilon, \delta)$-probabilistically differentially private, and let $\mu_x$ be the law of $A(x)$ on $(\calY, \calG)$. Let $k : \calY \times \calH \rightarrow [0, 1]$ be a probability transition kernel. Then, the algorithm $B : \calX \rightarrow \calZ$ where $B(x)$ has law $\eta_x$ given by
$$
\eta_x(dz) = \int_{\calY}k(dz, y)\mu_x(dy)
$$
is $(\epsilon, \delta)$-differentially private.
\end{lemma}

\begin{proof}
Let $x, x' \in \calX$ be neighboring inputs, and $\nu$ a finite measure on $(\calY, \calG)$ such that $\mu_x, \mu_{x'} << \nu$ \rrcomment{Double inequality typo?} (for instance, one could take $\nu = \mu_x + \mu_{x'}$). Let $g_x$ and $g_{x'}$ be the densities for $\mu_x$ and $\mu_{x'}$ respectively with respect to $\nu$. Let $G := \left\{ y \in \calY : \frac{g_x(y)}{g_{x'}(y)} > \epsilon\right\}$. Observe that, for any $E \in \calH$, we have
\begin{align*}
    \P(B(x) \in E) &=  \int_{\calY}\int_{E}k(dz, y)\mu_x(dy) = \int_{G^c}\int_{E}k(dz, y)\mu_x(dy) + \int_{G}\int_{E}k(dz, y)\mu_x(dy) \\
    &\leq \delta + \int_{G}\int_E k(dz, y)\mu_x(dy) = \delta + \int_G\int_E k(dz, y) g_x(y) \nu(dy) \\
    &\leq \delta + e^\epsilon \int_G\int_E k(dz, y) g_{x'}(y)\nu(dy) = \delta + e^\epsilon \int_G \int_E k(dz, y) \mu_{x'}(dy) \\
    &= e^\epsilon \P(B(x') \in E) + \delta.
\end{align*}
Which is exactly the desired result, so we are done.
\end{proof}

Post-processing of the form presented in Lemma~\ref{lem:clos_pp} can be interpreted in the following manner. Before beginning computation, for each possible outcome $y \in \calY$ of the computation, the data analyst selects some distribution of $\calZ$. In particular, this distribution depends in no way on the underlying database $x \in \calX$. After computing $A(x)$, the analyst then draws from the corresponding post-processing distribution, and releases that draw as the final, randomized output. 

This view on post-processing via transition kernels readily extends to the case of sequential interactions with private data. For our particular setting, there will be a sequence of transition kernels $(k^{(n)})_{n \in \N}$. The $n$th such kernel will can be viewed as a mapping $k^{(n)} : \calZ^{n - 1} \times \calY \times \calH \rightarrow [0, 1]$. The additional first argument can be viewed as the post-processed outputs of the first $n - 1$ algorithms. In other words, the exact distributions we choose to correspond to each possible outcome $y \in \calY$ for the $n$th round of computation depends on the underlying dataset $x \in \calX$ \textit{only} through the post-processed outputs of the first $n - 1$ rounds of computation. 

With this view of post-processing, we get the following more general lemma.

\begin{lemma}
\label{lem:clos_ppc}
Let $(A_n)_{n \in \N}$ and $(B_n)_{n \in \N}$ be sequences of algorithms, and for all $x \in \calX$, define the filtration $(\calF_n(x))_{n \in \N}$ given by $\calF_n(x) := \sigma(B_m(x) : m \leq n)$. For any any $x \in \calX$, $n \in \N$, let $\mu_x : \calG \times \calZ_{n - 1} \rightarrow [0, 1]$ be the conditional law of $A_n(x)$ given $B_{1:n - 1}(x)$, i.e. for all $z_1, \dots, z_{n - 1} \in \calY$,
$$
\P(A(x) \in G | B_{1:n-1}(x) = z_{1:n -1}) = \mu_x^{(n)}(G, z_{1: n -1}), \qquad \forall G \in \calG.
$$
In addition, assume $(k^{(n)})_{n \in \N}$ is a sequence of conditional transition kernels $k^{(n)} : \calH \times \calY \times \calZ^{n - 1} \rightarrow [0, 1]$ such that, for all $z_{1:n - 1} \in \calZ^{n - 1}, y \in \calY$
$$
\P(B_n(x) \in E | B_{1:n - 1}(x) = z_{1:n - 1}, A_n(x) = y) = k^{(n)}(E, y, z_{1:n -1}), \qquad \forall E \in \calH, \forall x \in \calX.
$$
Suppose $A_n$ is $(\epsilon_n, \delta_n)$-probabilistically differentially private given $\calF_{n - 1}(x)$. For $\epsilon > 0$ and $\delta = \delta' + \delta'' > 0$, let $N(\cdot)$ be the input-dependent stopping time defined in Theorem~\ref{thm:new_filter}. Then, the algorithm $B_{1:N(\cdot)}(\cdot) : \calX \rightarrow \calZ$ is $(\epsilon, \delta)$-differentially private.
\end{lemma}
\begin{proof}
Let $x \sim x'$ be arbitrary neighboring inputs in the space $\calX$. We assume that $\delta_n(x) = 0$ for all $n \in \N$, as the general case follows by conditioning in the same manner as in the proof of Theorem~\ref{thm:new_filter}. It suffices to check that $\P(B_{1:N(x)}(x) \in E) \leq e^\epsilon\P(B_{1:N(x')}(x') \in E)$, where $E = E_1 \times \cdots \times E_n \times \calY \times \calY \times \cdots$ is an arbitrary finite-dimensional rectangle. 

By Theorem~\ref{thm:filter_odom}, we know there is a ''good" set $\Omega_G \in \calF$ such that $\P(\Omega_G^c) \leq \delta'$ and $\calL_{1:N(x)}(x, x') \leq \epsilon$ on $\Omega_G$. Since
$$
\P(B_{1:N(x)}(x) \in E) = \P(B_{1:N(x)}(x) \in E, \Omega_G) + \P(B_{1:N(x)}(x) \in E, \Omega_G^c) \leq \P(B_{1:N(x)}(x) \in E, \Omega_G) + \delta',
$$
the result readily follows if we can demonstrate that $\P(B_{1:N(x)}(x) \in E, \Omega_G) \leq e^\epsilon \P(B_{1:N(x')}(x') \in E, \Omega_G)$. As such, let $G \subset \calY^\infty$ be the push-forward $B_{1:N(x)}(x)(\Omega_G)$ and $G_i$ the set of $i$th round outputs of $A_i(x)$ consistent with the outputs from the first $i - 1$ rounds, i.e.
$$
G_i := G_i(y_1, \dots, y_{i - 1}) := \left\{y_n : (y_{1:n}, \bar{y}_{n + 1:\infty}) \in G, \text{ some } \bar{y}_{n + 1:\infty} \in \calY^\infty\right\}.
$$

Now, let $\nu$ be a $\sigma$-finite reference measure on $(\calY, \calG)$ such that $\mu_x^{(n)}, \mu_{x'}^{(n)} << \nu$ for all $n \in \N$. Correspondingly, let $p^{(n)}_x, p^{(n)}_{x'}: \calY \times \calZ^{n - 1} \rightarrow \R_{\geq 0}$ be the corresponding conditional densities for $\mu_x^{(n)}$ and $\mu_{x'}^{(n)}$ respectively with respect to the dominating measure $\nu$. Letting $N' := N(x) \land n$, we consequently have:
\begin{align*}
    \P(B_{1:N(x)}(x) \in E, \Omega_G) &= \int_{G_1}\mu^{(1)}_x(dy_1)\int_{E_1}k^{(1)}(dz_1, y_1)\int_{G_2}\mu^{(2)}(dy_2, z_1) \int_{E_2}k^{(2)}(dz_2, y_2, z_1) \\ 
    &\cdots \int_{G_{N'}} \mu^{(N')}_x(dy_{N'})\int_{E_{N'}}k^{(N')}(dz_{N'}, y_{N'}, z_{1:N' - 1}) \\
    &= \int_{G_1}\nu(dy_1)p_x^{(1)}(y_1)\int_{E_1}k^{(1)}(dz_1, y_1)\int_{G_2}\nu(dy_2)p_x^{(2)}(y_2|z_1) \int_{E_2}k^{(2)}(dz_2, y_2, z_1) \\ 
    &\cdots \int_{G_{N'}} \nu(dy_{N'})p^{(N')}_x(y_{N'}|z_{1:N' - 1})\int_{E_{N'}}k^{(N')}(dz_{N'}, y_{N'}, z_{1:N' - 1}) \\
    &= \int_{G_1}\nu(dy_1)(y_1)\int_{E_1}k^{(1)}(dz_1, y_1)\int_{G_2}\nu(dy_2)\int_{E_2}k^{(2)}(dz_2, y_2, z_1) \\ 
    &\cdots \int_{G_{N'}} \nu(dy_{N'})\int_{E_{N'}}k^{(N')}(dz_{N'}, y_{N'}, z_{1:N' - 1})\prod_{i = 1}^{N'}p_x^{(i)}(y_i | z_{1:i - 1}) \\
    &\leq e^\epsilon\int_{G_1}\nu(dy_1)(y_1)\int_{E_1}k^{(1)}(dz_1, y_1)\int_{G_2}\nu(dy_2)\int_{E_2}k^{(2)}(dz_2, y_2, z_1) \\ 
    &\cdots \int_{G_{N'}} \nu(dy_{N'})\int_{E_{N'}}k^{(N')}(dz_{N'}, y_{N'}, z_{1:N' - 1})\prod_{i = 1}^{N'}p_{x'}^{(i)}(y_i | z_{1:i - 1}) \\
    &= e^\epsilon \P(B_{1:N(x')}(x') \in E, \Omega_G).
\end{align*}
In the above, the inequality $\prod_{i = 1}^{N'}p_x^{(i)}(y_i | z_{1:i - 1}) \leq e^\epsilon \prod_{i = 1}^{N'}p_{x'}^{(i)}(y_i | z_{1:i - 1})$ follows from the assumption of bounded privacy loss placed on the set $G$. Likewise, the last line follows from the fact that $N(x)$ only depends on $x$ through the values $A_{1:\infty}(x)$. Consequently, when $A_{1:\infty}(x) = y_{1:\infty} = A_{1:\infty}(x')$, we have $N(x) = N(x')$.

The result now follows because $\P(B_{1:N(x')}(x') \in E, \Omega_G) \leq \P(B_{1:N(x')}(x') \in E)$ by monotonicity.
\end{proof}

==> Old_Tex/zcdp.tex <==
\section{Generalization to zCDP}
\label{app:zcdp}
In this section, we prove an extension to Theorem~\ref{thm:fully_adaptive} that allows the algorithms being composed to either satisfy conditional differential privacy \textit{or} conditional zero-concentrated privacy with probability one (this is made precise in the theorem statement). We provide this relatively straightforward extension because the privacy loss of many common algorithms (in particular, Gaussian mechanisms) can be more tightly characterized by zero-concentrated differential privacy. 

Zero-concentrated differential privacy, constructed by~\cite{bun2016concentrated}, is a form of privacy that involves characterizing the uncentered moment generating function of the privacy loss random variable. For our purposes, the definition of zero-concentrated differential privacy is as follows.

\begin{definition}[Zero-concentrated differential privacy~\citep{bun2016concentrated}]
\label{def:zcdp}An algorithm $A$ is said to satisfy $\frac{1}{2}\epsilon^2$-zero-concentrated differential privacy (or $\frac{1}{2}\epsilon^2$-zCDP for short) if, for any $\lambda \geq 0$, we have
$$
\E\left( e^{\lambda \calL(x, x')}\right)  \leq e^{\frac{1}{2}\lambda(\lambda + 1)\epsilon_n^2}.
$$

\end{definition}

If we were considering zero-concentrated differentially private algorithms in isolation, the following would be a reasonable definition of conditional zCDP.

\begin{definition}[Conditional zCDP]
\label{def:czcdp}
Suppose $A$ and $B$ are algorithms having inputs in a space $\calX$ and outputs in measurable spaces $(\calY, \calG)$ and $(\calZ, \calH)$. Suppose $\epsilon: \calZ \rightarrow \R_{\geq 0}$ is measurable. We say the algorithm $A$ is $\frac{1}{2}\epsilon^2$-zCDP conditioned on $B$ if, for any neighboring datasets $x \sim x'$ and all $\lambda \geq 0$,
$$
\E\left(e^{\lambda \calL(x, x')} \mid B(x)\right) \leq e^{\frac{1}{2}\lambda(\lambda + 1)\epsilon(x)^2}.
$$



\end{definition}

Note that the constant $\lambda$ in Definition~\ref{def:czcdp} can also be taken to be a $B(x)$-measurable random variable, adding increased generality.

While Definition~\ref{def:czcdp} is a step in the right direction, what we actually want is a bit more subtle. In particular, in the context of adaptive data analysis, we want the data analyst to be able to select the type of privacy an algorithm satisfies on the fly. That is, given the outputs of the first $n - 1$ algorithms, the data analyst can \textit{then} decide whether to run an algorithm satisfying conditional DP or zCDP. The conditions of the following theorem establish precisely this desideratum. 

\begin{thm}
\label{thm:zcdp}
Let $(A_n)_{n \geq 1}$ be an adaptive sequence of algorithms, and, for any $x$, let $(\calF_n(x))_{n \in \N}$ be the natural filtration generated by $(A_n(x))_{n \in \N}$. For any $n \geq 1$, assume there are functions $\epsilon_n, \delta_n : \calY^{n - 1} \times \calZ^{n - 1} \rightarrow \R_{\geq 0}$. For any $x \sim x'$ neighbors and any $n \geq 1$, assume that with probability 1 we have either
\begin{enumerate}
    \item $\P(A_{1:n}(x) \in G \mid \calF_{n - 1}(x)) \leq e^{\epsilon_n(x)}\P(A_{1:n}(x') \in G \mid \calF_{n - 1}(x)) + \delta_n(x)$ for events $G$, or
    \item $\delta_n(x) = 0$ and $\E\left(e^{\lambda \calL_n(x, x')} \mid \calF_{n - 1}(x)\right) \leq e^{\frac{1}{2}\lambda(\lambda + 1)\epsilon_n(x)^2}$ for all $\lambda \geq 0$.
\end{enumerate}
Then, for any $\epsilon >0$ and $\delta = \delta' + \delta''$, letting $N$ be as outlined in Theorem~\ref{thm:fully_adaptive}, we have that the algorithm $A_{1:N(\cdot)}(\cdot)$ is $(\epsilon, \delta)$-differentially private.
\end{thm}

The assumptions on the algorithms in Theorem~\ref{thm:zcdp} essentially say that, with the information available up to time $n - 1$, the analyst will then select the mode of privacy of the next algorithm, either being DP or zCDP. As was the case for Theorem~\ref{thm:fully_adaptive}, it is first easier to prove the case where conditional differential privacy is replaced by conditional probabilistic differential privacy. As such, we start by proving the following lemma.

\begin{lem}
\label{lem:zcdp}
Theorem~\ref{thm:zcdp} holds when the first of two conditions is replaced by the stronger assumption that, for all neighbors $x \sim x'$,
$$
\P\left(\calL_n(x, x') > \epsilon_n(x) \mid \calF_{n - 1}(x)\right) \leq \delta_n(x).
$$
\end{lem}


\begin{proof}
We proceed using the same general approach as in Theorem~\ref{thm:new_filter}. That is, let $x \sim x'$ be fixed neighboring datasets, and assume that $\delta_n = 0$ for all $n \geq 1$. We let $(\calF_n(x))_{n \geq 1}$ be the natural filtration associated with $(A_n(x))_{n \geq 1}$.

If the first condition holds (that is, if $\P(\calL(x, x') > \epsilon_n(x) \mid \calF_{n - 1}(x)) = 0$), then applying Lemma~\ref{lem:priv_loss_bound} conditionally yields
$$
\E\left(e^{\lambda\calL_n(x, x')}\mid \calF_{n - 1}(x)\right) \leq e^{\frac{1}{2}\lambda(\lambda + 1)\epsilon_n(x)^2}.
$$
Thus, we see that the second condition actually holds for all algorithms being composed. Now, consider the process
$$
M_n := \sum_{m \leq n}\left\{\calL_n(x, x') - \frac{1}{2}\epsilon_n(x)^2\right\}.
$$
While $(M_n)_{n \in \N}$ itself is not in general a martingale with respect to $(\calF_n(x))_{n \in\N}$, from our above observation on the moment generating function of the privacy loss random variable, it follows that
$$
X_n := \exp\left(\frac{b}{a}M_n - \frac{b^2}{2a^2}\sum_{m \leq n}\epsilon_m(x)^2\right)
$$
is in fact a nonnegative supermartingale with respect to $(\calF_n(x))_{n \in \N}$. In particular, the proof of Theorem~\ref{fact:line_cross} found in Appendix~\ref{app:concentration} still goes through, yielding, for any $a, b > 0$, the concentration inequality
$$
\P\left(\exists n \in \N : M_n > \frac{b}{2} + \frac{b}{2a}\sum_{m \leq n}\epsilon_m(x)^2\right) \leq \exp\left(-\frac{b^2}{2a}\right).
$$
Optimizing over $a$ and $b$ as in the proof of Theorem~\ref{thm:new_filter} and then union bounding to handle the case of general $\delta_n$ yields the desired result.
\end{proof}
%Note that, like Lemma~\ref{thm:new_filter}, Lemma~\ref{lem:zcdp} can also be proved using the R\'enyi filters constructed by \citet{feldman2020individual}. 
Now we prove the main theorem of this appendix. \\

\begin{proof}[\textbf{Theorem~\ref{thm:zcdp}}]
This proof follows in a similar vein to the proof of Theorem~\ref{thm:fully_adaptive}. As such, let $x_0 \sim x_1$ be neighboring inputs. Define, for all $m \geq 1$, $A'_m$ to be the restricted algorithm, as outlined in the proof of Theorem~\ref{thm:fully_adaptive}. Let $(R_n)_{n \geq 1}$ be a sequence of algorithms such that on the event $E := \{\delta_n(A'_{1:n - 1}(b')) = 0\}$ we have that
$$
\P\left(R(b) \in \cdot \mid \calF_{n - 1}(x_{b'})\right) = \P\left(A'(b) \in \cdot \mid \calF_{n - 1}(x_{b'})\right)
$$
and on the complementary event $E^c := \{\delta_n(A'_{1:n - 1}(b')) > 0\}$ we have that $R_n$ is an instance of $(\epsilon_n, \delta_n)$-randomized response given $A'_{1:n - 1}$ (or, equivalently in terms of filtrations, given $\calF_{n - 1}$). It is straightforward to check that that there exist (random) transition kernels $(\rho_n)_{n \geq 1}$ such that
\begin{equation}
\label{eq:zcdp_meas}
\P\left(A'_n(b) \in \cdot \mid \calF_n(x_{b'})\right) = \rho^{(n)}_{b, b'}\left(\cdot \mid A'_{1:n - 1}(b')\right) \quad \text{almost surely},
\end{equation}
where $\rho_{b, b'}^{(n)} = \E\left(\rho_n(\cdot, R_n(b) \mid A'_{1:n -1}(b')) \mid A'_{1:n-1}(b')\right)$, the averaged conditional probability measure as defined in Footnote~\ref{foot:avg_cond}. On the event $E^c$ we can take $\rho_n = \nu_n$, where $\nu_n$ is as outlined in the proof of Theorem~\ref{thm:fully_adaptive} in Appendix~\ref{app:rand_resp}. On $E$ we can just take $\rho_n\left(\cdot, R_n(b) | A'_{1:n - 1}(b')\right) = \delta_{R_n(b)}$, where $\delta_y$ indicates the measure putting a point mass on $y \in \calY$. If follows from Equation~\ref{eq:zcdp_meas} that we can find an underlying probability space such that, for all $n \geq 1$, $A'_n(b)$ is equal to the random draws from $\rho_n(\cdot , R_n(b) \mid A'_{1: n - 1}(b'))$ almost surely. This, combined with the observation that the sequence of algorithms $(R_n)_{n \geq 1}$ satisfies the assumptions of Lemma~\ref{thm:zcdp}, allow the remainder of the proof to follow verbatim from the proof of Theorem~\ref{thm:fully_adaptive}.\end{proof}

